Only Pay for What Is Uncertain: Variance-Adaptive Thompson Sampling

Most bandit algorithms assume that the reward variances or their upper bounds are known, and that they are the same for all arms. This naturally leads to suboptimal performance and higher regret due to variance overestimation. On the other hand, underestimated reward variances may lead to linear regret due to committing early to a suboptimal arm. This motivated prior works on variance-adaptive frequentist algorithms, which have strong instance-dependent regret bounds but cannot incorporate prior knowledge on reward variances. We lay foundations for the Bayesian setting, which incorporates prior knowledge. This results in lower regret in practice, due to using the prior in the algorithm design, and also improved regret guarantees. Specifically, we study Gaussian bandits with {unknown heterogeneous reward variances}, and develop a Thompson sampling algorithm with prior-dependent Bayes regret bounds. We achieve lower regret with lower reward variances and more informative priors on them, which is precisely why we pay only for what is uncertain. This is the first result of its kind. Finally, we corroborate our theory with extensive experiments, which show the superiority of our variance-adaptive Bayesian algorithm over prior frequentist approaches. We also show that our approach is robust to model misspecification and can be applied with estimated priors.

==> 2bayes_unknown.tex <==
\section{Bayesian Setting with Unknown Variance}
\label{sec:bayes_unknown2}
%See \cref{sec:ng-prior} for the setting and problem parameterization.
In this section, we deal with the problem setup with unknown variance, as described in \cref{sec:prob}. We again propose a  thompson sampling (TS) based algorithm to obtain variance-adaptive bounds for this case as well, however the assumptions and posterior updates are non-trivial owning to the nature of unknown variance. The complete algorithm is described in \cref{sec: bayes_known_algo} below. Further our bayesian regret analysis for this case again shows a regret bound similar to roughly $\tilde O(\sqrt{2n} \sqrt{\sum_{i =1}^K\sigma_i^2 \log(1/\delta)})$, which again scales according to individual reward-variance of the $K$-arms (see \cref{thm:bayes_unknown2} for a more formal bound). 



\input{algo_bayes_unknown.tex}

\begin{restatable}[Regret Analysis: Adaptive-Variance Bounds for Unknown Variance]{thm}{bayesunknown}
\label{thm:bayes_unknown2}
%\red{Incomplete, don't read this}
Let $\bmu$ and $\bsigma^2$ respectively denotes the vector of arm means and variance in a $K$-armed Gaussian bandit that are generated as $(\mu_{i},1/\sigma_i^2) \sim P_* = NG(\mu_{0,i}(i), \kappa_{0,i}, \alpha_{0,i}, \beta_{0,i})$ for all $i \in [K]$ and the reward of arm-$i$, $Y_{i,s}$ is sampled from $\cN(\mu_{i},\sigma_i^2)$ ($\mu_{0,i},\kappa_{0,i},\alpha_{0,i},\beta_{0,i}$ being the known prior parameters). Then assuming $A^*$ be the optimal arm under $\bmu$ and $A_t$ be the pulled arm in round $t$ by TS, for any $\delta > 0$,

\begin{align*}
  &\E{\sum_{t = 1}^n \mu_{A^*} - \mu_{A_t}}
  \leq
  \\
  & \bigg[ \sqrt{n}  \sqrt{\E{\sum_{i = 1}^K  
  \biggsn{ 
  (1+2\beta_{0,i} 
    + 2\sigma_i^2\sqrt{\ln \frac{1}{\delta'}} + 2\ln \frac{1}{\delta'} + \kappa_{0,i} [(\bar{x}_{t,i} - \mu_{i})^2 + (\mu_{i} - \mu_{0,i})^2 ])\ln \bigg(1 + \frac{n}{2\alpha_{0,i}\kappa_{0,i}} \bigg)
    } \ln \frac{1}{\delta}}}\bigg]
  \,,
\end{align*}

where $c(\delta) = 2 \sqrt{2 (\kappa_{0}\sigma_0)^{-2} \log(1 / \delta)} K + \sqrt{2 \sigma_0^2 / \pi} K n \delta$ %\red{needs some correction}.
\end{restatable}

\begin{proof}
We start by noing that the posterior updates (from results of \cite{murphy2007conjugate}): 

\begin{align*}
    & \mu_{t,i} = \frac{\kappa_{0,i}\mu_{0,i} + N_t(i)\bar{x}_{t,i}}{\kappa_{0,i}+N_t(i)}
    \\
    & \kappa_{t,i} = \kappa_{0,i} + N_t(i)
    \\
    & \alpha_{t,i} = \alpha_{0,i} + N_t(i)/2
    \\
    & \beta_{t,i} = \beta_{0,i} 
    +
    \frac{1}{2}\sum_{t \in [T]}\1(A_t = i)(x_{t,i} - \bar{x}_{t,i})^2
    +
    \frac{\kappa_{0,i} N_t(i) (\bar{x}_{t,i} - \mu_{0,i})^2 }{2(\kappa_{0,i} + N_t(i))},
\end{align*}
where $N_t(i):= \sum_{s = 1}^{t-1} \1(A_t = i)$ denotes the number of pulls of arm $i$ up to round $t$, and $\bar x_{t,i}:= \frac{1}{N_t(i)}\sum_{s = 1}^{t-1} \1(A_t = i)Y_{t,i}$ being the averaged empirical mean reward of arm-$i$ at round $t$. 
%
Thus we have: 

\[
\mu_{i} - \hat \mu_{t,i}  \mid (\kappa_t,\lambda_t) \sim \cN(0 ,(\kappa_{t,i} \lambda_{t,i})^{-1},
\]
where $\lambda_{t,i} \sim \text{Gamma}(\alpha_{t,i},\beta_{t,i})$. 

Same as proof of \cref{thm:bayes_known}, we can break the regret in round $t$ as before:
\begin{align}
\label{eq:term5}
  \E{\mu_{A^*} - \mu_{A_t}}
  & = \E{\condE{\mu_{A^*} - \mu_{A_t}}{H_t}} \nonumber \\
  & = \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}} +
  \E{\condE{{{\hat{\mu}_{t,A_t}}}- \mu_{A_t}}{H_t}}\,,
  \nonumber \\
  & = \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}} +
  \mathbb E\Bigsn{\mathbb E_{\bsigma}\bigsn{\mathbb E [\hat{\mu}_{t,A_t}- \mu_{A_t} \mid \bsigma ] \mid H_t} }\,, \nonumber
  \\
  & = \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}} 
\end{align}

where $\sigma_{t,i}^2$ is defined as $\sigma_{t,i}^2:= \frac{1}{{\kappa_{t,i}\lambda_{t,i}}}$ which is a `sampled posterior variance', (where recall $\lambda_{t,i} \sim \text{Gam}(\alpha_{t,i},\beta_{t,i})$). The last equality holds since given $H_t$ and $\bsigma$,  $E[\mu_{i} \mid H_t] 
 = \hat{\mu}_{t,i}$ for any $i \in [K]$ by definition of the posterior update. %\red{check the argument}.

Now given $H_t$ and $\bsigma_t$, let us define $C_t(i) = \sqrt{2 \sigma_{t, i}^2 \log(1 / \delta)}$ -- the high-probability confidence interval of arm $i$ in round $t \in [K], ~\forall i \in [K]$. Now consider the event $E_t$:
\begin{align*}
  E_t
  = \set{\forall i \in [K]: \abs{\mu(i) -  \hat{\mu}_t(i)} \leq C_t(i)},
\end{align*}
which essentially indicates the `good event' when all the confidence intervals at round $t$ hold good. 
%

Further note, given $\cH_t$ and $\sigma_{i}^2$ (or equivalently $\lambda_{t,i})$),  $\mu_i - \hat{\mu}_{t,i} \mid \sigma_{t,i}^2, H_t \sim \cN(\mathbf{0}, \sigma_{t,i}^2)$, since $\sigma_t$ and $\sigma$ has same posterior. 
%\red{I am confused a bit}
Thus following same analysis as \eqref{eq:bayes regret scale}, we get: 
%So we w.h.p. $(1-\delta')$, we have \red{checK!}:

\begin{align}
  \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar{E}_t}}{\bsigma_t, H_t}
  & \leq \sum_{i = 1}^K \frac{1}{\sqrt{2 \pi \sigma_{t, i}^2}}
  \int_{x = C_t(i)}^\infty x
  \exp\left[- \frac{x^2}{2 \sigma_{t, i}^2}\right] \dif x \nonumber \\
  & = \sum_{i = 1}^K - \sqrt{\frac{\sigma_{t, i}^2}{2 \pi}}  \int_{x = C_t(i)}^\infty \frac{\partial}{\partial x}
  \left(\exp\left[- \frac{x^2}{2 \sigma_{t, i}^2}\right]\right) \dif x  \nonumber \\
  & = \sum_{i = 1}^K \sqrt{\frac{\sigma_{t, i}^2}{2 \pi}} \delta.
  \label{eq:bayes_regret_scale2}
\end{align}

Now note, using \eqref{eq:bayes_regret_scale2}, we get:

\begin{align}
 \label{eq:bayes_regret_scale3}
\mathbb{E}_{H_t,\bsigma}&\Bigsn{\mathbb{E}_{\bsigma_t}\bigsn{\E{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar{E}_t}\mid \bsigma_t} \mid H_t}} 
	\leq \nonumber 
    \sum_{i = 1}^K \mathbb{E}_{H_t,\bsigma}\Bigsn{ \mathbb E_{\bsigma_{t}}[ \sqrt{\frac{\sigma_{t,i}^2}{2 \pi}} \mid H_t,\bsigma } ]\delta
    \\
    & = \frac{1}{\sqrt{2 \pi}}\sum_{i = 1}^K \mathbb{E}_{H_t,\bsigma}\Bigsn{ \mathbb E_{\bsigma_{t}}[ \sigma_{t,i} \mid H_t,\bsigma ]}\delta
    \\
    & = \sum_{i = 1}^K \mathbb{E}_{H_t,\bsigma}\Bigsn{ \mathbb E_{\lambda_{t,i} \sim \text{Gam}(\alpha_{t,i},\beta_{t,i})}{ \sqrt{\frac{1}{2 \kappa_{t,i}\lambda_{t,i}\pi}}} }\delta \nonumber
    \\
    &
    \leq \sum_{i = 1}^K \frac{\delta}{\sqrt{2\pi}}\mathbb{E}_{H_t,\bsigma}\Bigsn{ \sqrt{\frac{1}{ \kappa_{t,i}}}  \sqrt{\mathbb E_{\lambda_{t,i}} \biggsn{\frac{1}{\lambda_{t,i}} } } } \nonumber
    \\
    &
    = \sum_{i = 1}^K \frac{\delta}{\sqrt{2\pi}} \mathbb{E}_{H_t,\bsigma}\Bigsn{ \sqrt{\frac{1}{ \kappa_{t,i}}}
    \sqrt{\frac{\beta_{t,i}}{ (\alpha_{t,i} -1)}   }},
\end{align}
where the last equality holds by the fact that given $H_t$, $\frac{1}{\lambda_{t,i}}$ follows the \textit{Inverse-Gamma}$(\alpha_{t,i},\beta_{t,i}^{-1})$ distribution and \cref{lem:inv_gam} \cite{cook08}. 
%

Now given any fixed $\bsigma$ and $\delta' \in (0,1)$, for any $t$, let us define an event, 
\[
\cG_{t} := \bigg\{ \forall i \in [K]:  \frac{1}{N_\tau(i)-1}\sum_{t = 1}^\tau\I{A_t = i} \frac{(x_{t,i} - \bar x_{\tau, i})^2}{\sigma_{i}^2} \leq 1 + 2\sqrt{\frac{\ln (1/\delta')}{N_\tau(i)-1}} + \frac{2\ln (1/\delta')}{N_\tau(i)-1} \bigg \}.
\]

Then the regret expression from \eqref{eq:term5} can be further decomposed as:
\begin{align}
\label{eq:term2}
  &\condE{{\hat{\mu}_{t,A^*}}  - \mu_{A^*}}{H_t} \nonumber
  \\  
  &\leq \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{E_t}}{H_t} +
  \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar{E}_t}}{H_t} \nonumber
  \\
  & = \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{E_t} \I{\cG_t}}{H_t} + \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{E_t} \I{\bar \cG_t}}{H_t}
  +\condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar{E}_t}}{H_t}\nonumber
  \\
  & \leq \condE{C_t(A^*)\I{\cG_t}}{H_t} + \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar \cG_t}}{H_t}
  +\condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar{E}_t}}{H_t}
  \,.
\end{align}

where the inequality follows from the observation that
\begin{align*}
  \condE{({\hat{\mu}_{t,A_t}} - \mu_{A_t}) \I{E_t}\I{\cG_t}}{H_t}
  \leq \condE{C_t(A_t)\I{\cG_t}}{H_t}\,.
\end{align*}

The remaining proof is to bounds the three terms of \eqref{eq:term2}.

{i. Bounding the third term in \eqref{eq:term2}:} This term can be bounded as in \eqref{eq:bayes_regret_scale3}. 

{ii. Bounding the second term in \eqref{eq:term2}:} For this term note that using \cref{lem:chi_conc}:
\begin{align*}
\condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar \cG_t}}{H_t} \leq \delta'
\end{align*}
%\red{need the max-bound}

{iii. Bounding the first term in \eqref{eq:term2}:} This case, we start by noting that 
\begin{align*}
\mathbb E_{\bmu, \bsigma, \bsigma_t}[C_t(A^*)\I{\cG_t} \mid H_t] =
\mathbb E_{\bsigma_t}[ \mathbb E_{\bmu, \bsigma} [C_t(A^*)\I{\cG_t} \mid \bsigma_t] \mid H_t] = \mathbb E_{\bsigma_t}[ \mathbb E_{\bmu, \bsigma} [C_t(A_t)\I{\cG_t} \mid \bsigma_t] \mid H_t], 
\end{align*}

where the last part follows from the fact that given $H_t$ and $\bsigma_t$, $A_t \mid H_t$ and $A^* \mid H_t$ have the same distributions. %\red{check, possibly conditioning on $\bsigma_t$ is redundant -- removed it}. 
%
Now we chain all inequalities for the regret in round $t$ and get:

\begin{align*}
  \E{\mu_{A^*} - \mu_{A_t}}
  \leq 2 \mathbb E_{H_t,\bmu,\bsigma}[C_t(A_t)] 
  + 
  \sum_{i = 1}^K \frac{\delta}{\sqrt{2\pi}} \mathbb{E}_{H_t,\bmu,\bsigma}\Bigsn{ \sqrt{\frac{1}{ \kappa_{t,i}}}
    \sqrt{\frac{\beta_{t,i}}{ (\alpha_{t,i} -1)}   }}\delta\,.
\end{align*}

Therefore, the $n$-round Bayes regret is bounded as
\begin{align*}
  \E{\sum_{t = 1}^n \mu_{A^*} - \mu_{A_t}}
  \leq 2 \mathbb E_{H_T,\bmu,\bsigma}[\sum_{t = 1}^n C_t(A_t)] 
  + 
  \sum_{t = 1}^n \sum_{i = 1}^K \frac{\delta}{\sqrt{2\pi}} \mathbb{E}_{H_T,\bmu,\bsigma}\Bigsn{ \sqrt{\frac{1}{ \kappa_{t,i}}}
    \sqrt{\frac{\beta_{t,i}}{ (\alpha_{t,i} -1)}   }}\delta\,.
\end{align*}


\begin{align*}
  &\E{\sum_{t = 1}^n C_t(A_t)}
  = \E{\sum_{t = 1}^n \sum_{i = 1}^K \1(A_t = i) C_t(i)} 
  = \E{\sum_{i = 1}^K \bigg[ \sum_{t = 1}^n \1(A_t = i) C_t(i) \bigg]}
  \\
  &\overset{(1)}{\leq} \E{\sum_{i = 1}^K \bigg[ \sqrt{N_n(i)} \sqrt{\sum_{t = 1}^n C_t^2(i)\1(A_t = i) }\bigg]}
  \\
  &\overset{(2)}{\leq} \E{ \bigg[ \sqrt{\sum_{i = 1}^K N_n(i)} \sqrt{\sum_{i = 1}^K \sum_{t = 1}^n C_t^2(i)\1(A_t = i) }\bigg]}
  \\
  &\overset{(3)}{\leq}  \bigg[ \sqrt{\sum_{i = 1}^K N_n(i)} \sqrt{\E{ \sum_{i = 1}^K \sum_{t = 1}^n C_t^2(i)\1(A_t = i) }\bigg]}
  \\
  &\overset{}{=}  \bigg[ \sqrt{n} \sqrt{\E{ \sum_{i = 1}^K \sum_{t = 1}^n C_t^2(i)\1(A_t = i) }\bigg]}
  \\
  & \overset{(4)}{\leq} \bigg[ \sqrt{n} \sqrt{{ \sum_{i = 1}^K \sum_{s = 1}^n E_{H_\tau,\bmu,\bsigma}\biggsn{
    \frac{\Bigsn{2\beta_{0,i} 
    +
    \sigma_i^2 (s-1)
    +
    \kappa_{0,i} [\frac{\sigma_{i}^2}{s} + (\mu_{i} - \mu_{0,i})^2  ]  }}
    {2(\kappa_{0,i} + s)(\alpha_{0,i} + s/2 -1)} \mid N_\tau(i)} }\bigg]}
  \\
  & \leq \bigg[ \sqrt{n} \sqrt{\E{ \sum_{i = 1}^K \sum_{t = 1}^n C_t^2(i)\1(A_t = i) }\bigg]}
  \\
  %%
\end{align*}

where $(1)$ and $(2)$ uses Cauchy-Schwarz, $(2)$ applies Jensen's inequality, the Inequality $(4)$ above follows from \cref{lem:gam_conc}, and the second last inequality follows from \cref{lem:reciprocal sum}.

\iffalse %%%%%%%%%%%%%%%

&\overset{(4)}{\leq}  \E{\sum_{i = 1}^K \bigg[ \sqrt{N_n(i)}  \sqrt{\sum_{s = 1}^n  
  \biggsn{ 
  \frac{2\beta_{0,i} 
    +
    \sigma_i^2(s-1 + 2\sqrt{\ln \frac{1}{\delta'}(s-1)} + 2\ln \frac{1}{\delta'})
    +
    \kappa_{0,i} [(\bar{x}_{t,i} - \mu_{i})^2 + (\mu_{i} - \mu_{0,i})^2  ]  }{(\kappa_{0,i} + s)(2\alpha_{0,i} + s - 2)}
  } \ln \frac{1}{\delta}\1(A_t = i)}}\bigg]
  \\ 
  &\leq \E{\sum_{i = 1}^K \bigg[ \sqrt{N_n(i)}  \sqrt{  
  \biggsn{ 
  (1+2\beta_{0,i} 
    + 2\sqrt{\ln \frac{1}{\delta'}} + 2\ln \frac{1}{\delta'} + \kappa_{0,i} [(\bar{x}_{t,i} - \mu_{i})^2 + (\mu_{i} - \mu_{0,i})^2 ])\ln \bigg(1 + \frac{n}{2\alpha_{0,i}\kappa_{0,i}} \bigg)
    } \ln \frac{1}{\delta}}}\bigg]
    \\
    &\leq \bigg[ \sqrt{n}  \sqrt{\E{\sum_{i = 1}^K  
  \biggsn{ 
  (1+2\beta_{0,i} 
    + 2\sqrt{\ln \frac{1}{\delta'}} + 2\ln \frac{1}{\delta'} + \kappa_{0,i} [(\bar{x}_{t,i} - \mu_{i})^2 + (\mu_{i} - \mu_{0,i})^2 ])\ln \bigg(1 + \frac{n}{2\alpha_{0,i}\kappa_{0,i}} \bigg)
    } \ln \frac{1}{\delta}}}\bigg]

\red{old bound with precision lower bounds - reject below!}

\begin{align*}
  \E{\sum_{t = 1}^n C_t(A_t)}
  & = \E{\sum_{t = 1}^n \sum_{i = 1}^K \1(A_t = i) C_t(i)} 
  = \E{\sum_{i = 1}^K \bigg[ \sum_{t = 1}^n \1(A_t = i) C_t(i) \bigg]}
  \\
  &\leq \E{\sum_{i = 1}^K \bigg[ \sqrt{N_t(i)} \sqrt{\sum_{t = 1}^n C_t^2(i)\1(A_t = i) }\bigg]}
  \\
  &=  \E{\sum_{i = 1}^K \bigg[ \sqrt{N_t(i)}  \sqrt{\sum_{t = 1}^n \frac{1}{\lambda_{0,i}\big(\kappa_{0,i} + n\big)} \log(1 / \delta)\1(A_t = i)}\bigg]}
  \\
  &=  \E{\sum_{i = 1}^K \bigg[ \sqrt{2N_t(i)\lambda_{0,i}^{-1}}  \sqrt{\sum_{s = 1}^{N_n(i)} \frac{1}{\kappa_{0,i} + s} \log(1 / \delta) + \frac{1}{\kappa_{0,i}}\log(1/\delta)}\bigg]}
  \\
  &\leq \E{\sum_{i = 1}^K \bigg[ \sqrt{2N_t(i)(\lambda_{0,i}^{-1})}  \sqrt{\sum_{s = 1}^{n} \frac{1}{\kappa_{0,i} + s} \log(1 / \delta) + \frac{1}{\kappa_{0,i}}\log(1/\delta)}\bigg]}
  \\	  
  & \overset{(a)}{\leq} \E{\sum_{i = 1}^K \bigg[ \sqrt{2N_t(i)\lambda_{0,i}^{-1}}  \sqrt{\Big(\log(1 + n\kappa_{0,i}) + \frac{1}{\kappa_{0,i}}\Big)\log(1/\delta)}\bigg]}
  \\
  &= \E{\sum_{i = 1}^K \bigg[ \sqrt{2N_t(i)}  \sqrt{\lambda_{0,i}^{-1}\Big(\log(1 + n\kappa_{0,i}) + \frac{1}{\kappa_{0,i}}\Big)\log(1/\delta)}\bigg]}
  \\
  & \leq  \sqrt{2n} \sqrt{\sum_{i =1}^K\lambda_{0,i}^{-1}\Big(\log(1 + n\kappa_{0,i}) + \frac{1}{\kappa_{0,i}}\Big)\log(1/\delta)}
  \,.
\end{align*}
\fi %%%%%%%%%%%%%%%%%%%%%

\end{proof}




\iffalse %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Since $\lambda \sim Gamma(\alpha_{0,i},\beta_{0,i})$, we have:

\red{not true if $\lambda_{0,i} \geq $ (mode)}

\begin{align*}
	P(\I{\bar F}) \leq \lambda_{0,i} f(\lambda_{0,i}) & \leq \delta' 
	\\
	\implies &
	\frac{\beta_{0,i}^{\alpha_{0,i}}}{\Gamma(\alpha_{0,i}) }\lambda_{0,i}^{\alpha_{0,i}} e^{-\beta_{0,i} \lambda_{0,i}} \leq \delta'
	\\
	\implies & 
	\log\big( \frac{\beta_{0,i}^{\alpha_{0,i}}}{\Gamma(\alpha_{0,i}) }\big) + \alpha_{0,i}\log \lambda_{0,i} - \lambda_{0,i}\beta_0 \leq \log (\delta')
	\\
	\implies &
	\lambda_{0,i} \geq \frac{1}{\beta_{0,i}}\log \bigg( \frac{\beta_{0,i}^{\alpha_{0,i}}}{\Gamma(\alpha_{0,i}) \delta'} \bigg) + \frac{\alpha_{0,i}}{\beta_{0,i}} \log \lambda_{0,i} 
\end{align*}

We can now choose $\lambda_{0,i}$ based on Lem 18 of \cite{SKM21}
\fi %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsubsection{Additional Claims used in the Proof of \cref{thm:bayes_unknown2}} 

\begin{restatable}[\cite{cook08}]{lem}{invgam}
\label{lem:inv_gam}
Suppose $X$ follows a Gamma$(\alpha,\beta)$ distribution with shape parameter $\alpha>0$ and rate parameter $\beta > 0$, then $1/X$ follows an Inverse-Gamma$(\alpha,1/\beta)$ distribution. 
\\
Moreover if $\alpha>1$, $E[1/X] = \frac{\beta}{\alpha-1}$. 
\end{restatable}


\begin{restatable}[\cite{cook08}]{lem}{avgchi}
\label{lem:avg_chi}
Let ${\displaystyle X_{1},...,X_{n}}$ are i.i.d. ${\displaystyle N(\mu ,\sigma ^{2})}$ random variables, (a). then 
\[
{\displaystyle \sum _{i=1}^{n}\frac{(X_{i}-{\bar {X}_n})^{2}}{\sigma ^{2}}\sim \chi _{n-1}^{2}},
\]
where ${\displaystyle {\bar {X}_n}={\frac {1}{n}}\sum _{i=1}^{n}X_{i}}$ is the sample mean of $n$ random draws, and $\chi_{d}^2$ is the chi-squared random variable with $d$-degrees of freedom (for any $d \in \N_+$). 
\\
(b). Further if $X \sim \chi_d^2$, then $E[X] = d$.
\end{restatable}

\begin{restatable}[]{lem}{varbdd}
\label{lem:var_bdd}
For any $i \in [K]$, and round $\tau \in [T]$,
\begin{align*}
  E_{H_\tau,\bmu,\bsigma}&\biggsn{\frac{\beta_{\tau,i}}{ (\kappa_{\tau,i})(\alpha_{\tau,i} -1)} \mid N_{\tau,i}} 
    \leq  
        E_{H_\tau,\bmu,\bsigma}\biggsn{
    \frac{\Bigsn{2\beta_{0,i} 
    +
    \sigma_i^2 (N_{\tau}(i)-1)
    +
    \kappa_{0,i} [\frac{\sigma_{i}^2}{N_{t,i}} + (\mu_{i} - \mu_{0,i})^2  ]  }}
    {2(\kappa_{\tau,i})(\alpha_{0,i} + N_{\tau}(i)/2 -1)} \mid N_\tau(i)}
\end{align*}
\end{restatable}

\begin{proof}
We start by noting that for any $i \in [K]$, 
\begin{align*}
 \mathbb{E}_{H_\tau,\bsigma}&\Bigsn{ \mathbb E_{\bsigma_{\tau}}[ \sigma_{\tau,i} \mid H_{\tau},\bsigma ]}
	\\
	& = 
 \mathbb{E}_{H_{\tau},\bsigma}\Bigsn{ \mathbb E_{\lambda_{\tau,i} \sim \text{Gam}(\alpha_{\tau,i},\beta_{\tau,i})}{ \sqrt{\frac{1}{ \kappa_{\tau,i}\lambda_{\tau,i}}}} \mid H_{\tau},\bsigma}
    \\
    &
    \leq \mathbb{E}_{H_{\tau},\bsigma}\Bigsn{ \sqrt{\frac{1}{ \kappa_{\tau,i}}}  \sqrt{\mathbb E_{\lambda_{\tau,i}} \biggsn{\frac{1}{\lambda_{\tau,i}} } } \mid H_{\tau},\bsigma} 
    \\
    &
    = \mathbb{E}_{H_{\tau},\bsigma}\Bigsn{ \sqrt{\frac{1}{ \kappa_{\tau,i}}}
    \sqrt{\frac{\beta_{\tau,i}}{ (\alpha_{\tau,i} -1)}   } \mid H_{\tau},\bsigma},
\end{align*}
where the last equality holds by the fact that given $H_{\tau}$, $\frac{1}{\lambda_{t,i}}$ follows the \textit{Inverse-Gamma}$(\alpha_{\tau,i},\beta_{\tau,i}^{-1})$ distribution and \cref{lem:inv_gam} \cite{cook08}. Now from the posterior update rules, given $H_{\tau}$ we have:
\begin{align*}
\frac{\beta_{\tau,i}}{ (\alpha_{\tau,i} -1)} 
    & \leq 
    \frac{\beta_{0,i} 
    +
    \frac{1}{2}\sum_{t \in [\tau]}\1(A_t = i)(x_{t,i} - \bar{x}_{\tau,i})^2
    +
    \frac{\kappa_{0,i} N_t(i) (\bar{x}_{\tau,i} - \mu_{0,i})^2 }{2(\kappa_{0,i} + N_{\tau}(i))} }{(\alpha_{0,i} + N_{\tau}(i)/2 -1)}
    \\
    & \leq 
    \frac{2\beta_{0,i} 
    +
    \sum_{t \in [\tau]}\1(A_t = i)(x_\tau(i) - \bar{x}_{\tau,i})^2
    +
    \kappa_{0,i} [(\bar{x}_{\tau,i} - \mu_{i})^2 + (\mu_{i} - \mu_{0,i})^2  ]  }
    {2(\alpha_{0,i} + N_{\tau}(i)/2 -1)}
\end{align*}

Now given any fixed reward-precision $\lambda_i \sim \text{Gam}(\alpha_{0,i},\beta_{0,i})$, $\sigma_{i}^2:= \frac{1}{\lambda_{i}}$, mean-reward $\mu_i \sim \cN(\mu_{0,i},\sigma_{0,i}^2)$, and fixed number of pulls $N_\tau(i) = s$ (say), note $x_{t,i} \overset{iid}{\sim} \cN(\mu_{i}, \sigma_{i}^2)$ can be seen as $N_\tau(i) = s$ independent and identical draws from $\cN(\mu_i,\sigma_i^2)$. Thus
$\sum_{t = 1}^\tau\I{A_t = i} \frac{(x_{t,i} - \bar x_{\tau,i})^2}{\sigma_{i}^2} = \sum_{t = 1}^s\frac{(x_{t,i} - \bar x_{\tau,i})^2}{\sigma_{i}^2}$ follows $\chi^2(s-1)$, i.e. chi-squared distribution with $s-1$ degrees of freedom (see \cref{lem:avg_chi}). Further using \cref{lem:avg_chi}, part-(b) again, we know 
\[
E_{x_{t,i} \sim \cN(\mu_i,\sigma_i^2)} \biggsn{\sum_{t = 1}^s\frac{(x_{t,i} - \bar x_{\tau,i})^2}{\sigma_{i}^2}} = (s-1).
\]

Applying this to above chain of equations, note we get:

\begin{align*}
& E_{H_\tau,\bmu,\bsigma}\biggsn{\frac{\beta_{\tau,i}}{ (\kappa_{\tau,i})(\alpha_{\tau,i} -1)} \mid N_{\tau}(i)}
	\\    
    & = 
    E_{H_\tau,\bmu,\bsigma}\biggsn{
    \frac{{2\beta_{0,i} 
    +
    E_{x_{t,i}\sim \cN(\mu_i,\sigma_i^2)}\biggsn{\sigma_i^2 \sum_{t = 1}^{N_{\tau}(i)}(\frac{x_{t,i} - \bar{x}_{\tau,i}}{\sigma_i})^2 \mid \mu_i, \sigma_{i}}
    +
    \kappa_{0,i} [(\bar{x}_{\tau,i} - \mu_{i})^2 + (\mu_{i} - \mu_{0,i})^2  ]  }}
    {2(\kappa_{\tau,i})(\alpha_{0,i} + N_{\tau}(i)/2 -1)} \mid N_\tau(i)}
    \\
    & = 
    E_{H_\tau,\bmu,\bsigma}\biggsn{
    \frac{\Bigsn{2\beta_{0,i} 
    +
    \sigma_i^2 (N_{\tau}(i)-1)
    +
    \kappa_{0,i} \big[E_{\bar x_{\tau,i} \overset{\text{iid}}{\sim} \cN(\mu,\sigma^2/N_\tau(i))}[(\bar{x}_{\tau,i} - \mu_{i})^2 \mid \mu_i,\sigma_i] + (\mu_{i} - \mu_{0,i})^2  \big]  }}
    {2(\kappa_{\tau,i})(\alpha_{0,i} + N_{\tau}(i)/2 -1)} \mid N_\tau(i)}
    \\
    & \overset{(1)}{=} 
    E_{H_\tau,\bmu,\bsigma}\biggsn{
    \frac{\Bigsn{2\beta_{0,i} 
    +
    \sigma_i^2 (N_{\tau}(i)-1)
    +
    \kappa_{0,i} [\frac{\sigma_{i}^2}{N_{t,i}} + (\mu_{i} - \mu_{0,i})^2  ]  }}
    {2(\kappa_{\tau,i})(\alpha_{0,i} + N_{\tau}(i)/2 -1)} \mid N_\tau(i)}
\end{align*}
where (1) again follows since given $\mu_i, \sigma_i$ and $N_\tau(i)$ as before, $x_{t,i} \overset{\text{iid}}{\sim} \cN(\mu,\sigma^2)$, and thus by definition 
$\bar x_{\tau, i} = \frac{1}{N_{\tau}(i)} \sum_{t = 1}^\tau \I{A_t = i} x_{t,i} \sim \cN\big(\mu, \frac{\sigma^2}{N_{\tau}(i)}\big)$> This leads to $E_{\bar x_{\tau,i} \overset{\text{iid}}{\sim} \cN(\mu,\sigma^2/N_\tau(i))}[\bar x_{\tau, i} - \mu_i]^2 = \frac{\sigma_i^2}{N_{\tau}(i)}$. Thus the claim is concluded. 
\end{proof}
%Also further note that, given any fixed $\bsigma$ s.t. $\sigma_i^2:= 1/\lambda_i$ where $\lambda_i \sim \text{Gam}(\alpha_{0,i},\beta_{0,i})$.

\iffalse%%%%%%%%%%%%%%%%%%

\begin{restatable}[\red{chi-sqr confidence, not used} Lemma 1, \cite{massart}]{lem}{chiconc}
\label{lem:chi_conc}
Suppose $X$ is a chi-squared distribution with $D$ degrees of freedom, for some $D \in \N_+$, then for any $\delta \in (0,1)$, with probability at least $1-\delta$,
\begin{align*}
   X \leq D + 2\sqrt{{D\ln (1/\delta)} } + 2\ln (1/\delta)
\end{align*}
\end{restatable}


\begin{restatable}[\red{not used, needed if use precision lower bound}]{lem}{preclb}
\label{lem:prec_lb}
Let $X \sim Gamma(\alpha,\beta)$. Then given any $\delta \geq \frac{1}{\exp(\alpha)}$, w.h.p. at least $(1-\delta)$,
\[
X > \frac{\alpha}{e \beta}
\]
\end{restatable}


\begin{proof}
We start by noting that, for any $x_0 \in R_+$ and some $t>0$, applying Markov's Inequality we get:

\begin{align*}
\P(X < x_0) & = \P(-tX > -tx_0) = \P(\exp(-tX) > \exp(-x_0))
\\
& = \frac{\E{\exp(-tX)}}{\exp(-tx_0)}.
\end{align*}

Moreover, using gamma-pdf, we get:
\begin{align*}
\E{\exp(-tX)} & = \frac{\beta^\alpha}{\Gamma(\alpha)}\int_{x = 0}^{\infty}\exp(-tX)\exp(-\beta X)x^{\alpha -1}dx 
= \frac{\beta^\alpha}{\Gamma(\alpha)}\int_{x = 0}^{\infty}\exp(-(t+\beta)x)x^{\alpha -1}dx 
\\
& = \frac{\beta^\alpha}{\Gamma(\alpha)}\int_{u = 0}^{\infty}\exp(-u)\biggn{\frac{u}{t+\beta}}^{\alpha -1}\frac{du}{t+\beta}
\\
& = \frac{\beta^\alpha}{\Gamma(\alpha) (t+\beta)^\alpha}\int_{u = 0}^{\infty}\exp(-u)u^{\alpha-1}du = \frac{\beta^\alpha}{(t+\beta)^\alpha}.
\end{align*}

Since we want $\P(X < x_0) < \delta$, the goal is to find the threshold $x_0$  such that: 
\begin{align*}
\min_{t} \frac{\beta^\alpha \exp(tx_0)}{(t+\beta)^\alpha} < \delta.
\end{align*}

It is easy to check the minimum of the above expression is attained at $t = \frac{\alpha}{x_0} - \beta$, given $x_0 < \frac{\alpha}{\beta}$ since by definition we need $t>0$.

Combining the above two equations, we get:
\begin{align*}
\bigg(\frac{\beta}{\alpha}\bigg)^{\alpha} \frac{e^{\alpha - \beta x_0}}{x_0^\alpha} < \delta,
\end{align*}

 which implies to choose $x_{0}$ such that:

\[
x_0 \geq \frac{\alpha}{\beta} + \frac{\alpha}{\beta}\ln\Big( x_{0} \frac{\beta}{\alpha} \Big) + \frac{\ln (1/\delta)}{\beta} \text{ s.t. } x_{0} > \frac{\alpha}{\beta}.
\]

Finally, the claim holds noting that the above implies we can choose $x_0$ to be $\frac{\alpha}{e\beta}$, which satisfies the above inequality as long as $\ln (1/\delta) \leq \alpha$.

\iffalse%%%%%%%%%%%%%%%%
Or more loosely, it is enough to choose $x_0$ such that:

\[
x_0 \geq 1 + \frac{\ln (1/\delta)}{\beta} + \frac{\alpha}{\beta}\ln x_0 \text{ s.t. } x_{0} > \frac{\alpha}{\beta}.
\]

Finally note that above can be satisfied for any $x_0 > 2\bign{ 1 + \frac{\ln 1/\delta}{\beta} + \big(\frac{\alpha}{\beta}\big)^2 }$
by \cref{lem:tvslogt} where in our case $A = 1 + \frac{\ln 1/\delta}{\beta}$ and $B = \frac{\alpha}{\beta}$.
\fi %%%%%%%%%%%%%%%%%%%%%%%%
%We finally note that above can be satisfied setting $x_{0} = \frac{\alpha}{e \beta}$, which satisfies the above relation assuming $\alpha/e \geq \ln(1/\delta)$. 
\end{proof}

\begin{restatable}[(\red{Ignore - Not Used})]{lem}{tvslogt}
\label{lem:tvslogt}
For any $x > 0$ and $A> 0, B > 1$, $x > A + B\ln x$ for any $x \ge 2A + 2B^2$.
\end{restatable}

\begin{proof}
This follows from the calculation as shown below:
\begin{align*}
	A + B\ln x & = A + B\ln (2A + 2B^2 )\\
	& < A + B\ln\big(2B^2 (1 + A/B^2)\big)\\
	& < A + B\ln 2B^2 + A/B ~~~~\text{as } \ln(1+x) \leq x\\	
	& = A + A/B + 2B^2\\
	& \le 2A + 2B^2 = x,
\end{align*}
where the last inequality follows since $B > 1$.
\end{proof}

\fi%%%%%%%%%%%%%%%%%%%%%%%

==> BMTR.tex <==
\section{Bayesian Multi-Task Regression}
\label{sec:bayesian multi-task regression}

Multi-task Bayesian regression was proposed by \citet{lindley72bayes}. In their work, there is only one prior for all the regression tasks. In other words, there is no meta-prior and the posterior is calculated only for $2$ levels. In our work, we extended this formulation by adding a meta-prior. Now we need to compute the posterior across $3$ levels, which we work out in this section. Recall that all variances in our hierarchical data generation process are known. Formally, we have the following generative model
\begin{equation}
\begin{aligned}
  \theta_0 \;
  &\sim \; \mathcal{N}(\mu_0, \Lambda_0^{-1}) \\
  \theta_{t}|\theta_0 \;
  &\sim \; \mathcal{N}(\theta_0, \Sigma) \qquad\;\, \text{ for } t=1,2,\dots,T \\
  y_{t,i}|\theta_t, x_{t,i} \;
  &\sim \; \mathcal{N}(x_{t,i}^T \theta_t, \sigma^2) \quad \text{ for } i=1,2,\dots,N
\end{aligned}
\end{equation}
For convenience, we group all observations in a matrix-vector form as $X_t = (x_{t,1},\dots,x_{t,n})$ and $y_t = (y_{t,1},\dots,y_{t,n})$. Our goal is to compute $p\left(\theta_0 \middle| X_{1:T}, y_{1:T}\right)$. We begin by trying to recursively compute
\begin{equation}
  p(\theta_0|X_{1:t}, y_{1:t})
  \propto p(\theta_0|X_{1:t-1}, y_{1:t-1}) p(y_{t} | \theta_0, X_{t})
  \label{eq:recurse}
\end{equation}


\subsection{Computing $p(y_{t} | \theta_0, X_{t})$}

Note that, given $\theta_t$ and $X_t$, we have
\begin{equation}
    y_t = X_t\theta_t + \epsilon \qquad \text{ where } \epsilon \sim \mathcal{N}(0, \sigma^2 I)
\end{equation}
Similarly, given $\theta_0$, we have
\begin{equation}
    \theta_t = \theta_0 + \nu \qquad \text{ where } \nu \sim \mathcal{N}(0, \Sigma)
\end{equation}
Combining the above two equations
\begin{equation}
    y_t = X_t\theta_0 + X_t \nu + \epsilon
\end{equation}
From the above, it is clear that $y_t|\theta_0, X_{t}$ is a Gaussian. We can find the parameters of this distribution easily as
\begin{equation}
\begin{aligned}
    \mathbb{E}[y_t|\theta_0, X_t] &= X_t\theta_0\\
    \text{Cov}(y_t|\theta_0, X_t) &= \mathbb{E}[(y_t-X_t\theta_0)(y_t-X_t\theta_0)^T] \\
    &= \mathbb{E}[(X_t \nu + \epsilon)(X_t \nu + \epsilon)^T] \\
    &= \mathbb{E}[(X_t \nu\nu^TX_t^T + \epsilon \nu^T X_t^T + X_t \nu \epsilon^T + \epsilon\epsilon^T)] \\
    &= X_t \underbrace{\mathbb{E}[\nu\nu^T]}_{=\Sigma}X_t^T + \underbrace{\mathbb{E}[\epsilon \nu^T]}_{=0 \text{ as } \epsilon \perp \nu} X_t + X_t \underbrace{\mathbb{E}[\nu \epsilon^T]}_{=0 \text{ as } \epsilon \perp \nu} + \underbrace{\mathbb{E}[\epsilon\epsilon^T]}_{=\sigma^2 I} \\
    &= X_t\Sigma X_t^T + \sigma^2I
\end{aligned}
\end{equation}
Thus we get
\begin{equation}
    y_{t} | \theta_0, X_{t} \; \sim \; \mathcal{N}(X_t\theta_0, \  \sigma^2I + X_t\Sigma X_t^T)
    \label{eq:marginal_final}
\end{equation}


\subsection{Computing $p(\theta_0|X_{1:t}, y_{1:t})$ by induction}

\paragraph{Induction hypothesis:} $\forall t: \theta_0|X_{1:t}, y_{1:t} \; \sim \; \mathcal{N}(\mu_t, \Lambda_t^{-1}) $

\paragraph{Base case $t=0$:} This corresponds to prior as there is no data and thus by definition $\theta_0 \; \sim \; \mathcal{N}(\mu_0, \Lambda_0^{-1})$.

\paragraph{Inductive step} We derive the distribution of $\theta_0|X_{1:t}, y_{1:t}$ given that $\theta_0|X_{1:t-1}, y_{1:t-1} \; \sim \; \mathcal{N}(\mu_{t-1}, \Lambda_{t-1}^{-1})$. Then by using the recurrence from \eqref{eq:recurse} and marginal distribution from \eqref{eq:marginal_final}, we obtain
\begin{equation}
\begin{aligned}
    p(\theta_0|X_{1:t}, y_{1:t}) &\propto p(\theta_0|X_{1:t-1}, y_{1:t-1}) p(y_{t} | \theta_0, X_{t}) \\
    &\propto \exp\left\{ -\frac{1}{2} (\theta_0-\mu_{t-1})^T\Lambda_{t-1}(\theta_0-\mu_{t-1})  \right\}  \exp\left\{ -\frac{1}{2} (y_t-X_t\theta_0)^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}(y_t-X_t\theta_0)  \right\} \\
    &\propto \exp\left\{ -\frac{1}{2} (\theta_0-\mu_{t-1})^T\Lambda_{t-1}(\theta_0-\mu_{t-1})   -\frac{1}{2} (y_t-X_t\theta_0)^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}(y_t-X_t\theta_0)  \right\} \\
    &\propto \exp\left\{ -\frac{1}{2}\theta_0^T\Lambda_{t-1}\theta_0 +\theta_0^T\Lambda_{t-1}\mu_{t-1} - \frac{1}{2} \theta_0^TX_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}X_t\theta_0 + \theta_0^TX_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}y_t \right\} \\
    &\propto \exp\left\{ -\frac{1}{2}\theta_0^T\underbrace{\left(\Lambda_{t-1} + X_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}X_t\right)}_{=\Lambda_t}\theta_0 +\theta_0^T\underbrace{\left(\Lambda_{t-1}\mu_{t-1} + X_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}y_t \right)}_{=\Lambda_t\mu_t} \right\} \\
    &\propto \exp\left\{ -\frac{1}{2}\theta_0^T\Lambda_t\theta_0 +\theta_0^T\Lambda_t\mu_t \right\} \\
    &\propto \exp\left\{ -\frac{1}{2}\theta_0^T\Lambda_t\theta_0 +\theta_0^T\Lambda_t\mu_t -\frac{1}{2}\mu_t^T\Lambda_t\mu_t  \right\} \\
    &\propto \exp\left\{ -\frac{1}{2}(\theta_0-\mu_t)^T\Lambda_t(\theta_0-\mu_t) \right\} \\
\end{aligned}
\end{equation}
This completes our proof by induction, as now we have shown that $\theta_0|X_{1:t}, y_{1:t} \; \sim \; \mathcal{N}(\mu_t, \Lambda_t^{-1})$, where
\begin{equation}
\begin{aligned}
    \Lambda_t &= \Lambda_{t-1} + X_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}X_t\\
    \mu_t &= \Lambda_t^{-1} \left(\Lambda_{t-1}\mu_{t-1} + X_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}y_t \right)
\end{aligned}
\end{equation}
Using these recurrences, the posterior after $T$ tasks is a Gaussian with parameters
\begin{equation}
\begin{aligned}
    \Lambda_T &= \Lambda_0 + \sum_{t=1}^T X_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}X_t\\
    \mu_T &= \Lambda_T^{-1} \left( \Lambda_{0}\mu_{0} + \sum_{t=1}^T X_t^T(\sigma^2I + X_t\Sigma X_t^T)^{-1}y_t \right)
\end{aligned}
\end{equation}
In a high-dimensional setting, where $N<K$, the above equation is efficient as it handles matrices of size $N \times N$ at cost $O(N^{\omega})$. In a large-sample setting, where $K<N$, using $N \times N$ matrices can be costly. To reduce the computational cost to $O(K^{\omega})$, we apply the Woodbury matrix identity
\begin{equation}
  \left(A+UCV\right)^{-1}
  = A^{-1}-A^{-1}U\left(C^{-1}+VA^{-1}U\right)^{-1}VA^{-1}
\end{equation}
to $(\sigma^2I + X_t\Sigma X_t^T)^{-1}$. This yields new recurrences
\begin{equation}
\begin{aligned}
    \Lambda_t &= \Lambda_{t-1} + \frac{S_t}{\sigma^{2}} - \frac{S_t}{\sigma^{2}} \left(\Sigma^{-1}+ \frac{S_t}{\sigma^{2}}\right)^{-1} \frac{S_t}{\sigma^{2}}\\
    \mu_t &= \Lambda_t^{-1} \left(\Lambda_{0}\mu_{0} + \sum_{t=1}^T \frac{c_t}{\sigma^{2}} - \frac{S_t}{\sigma^{2}} \left(\Sigma^{-1}+ \frac{S_t}{\sigma^{2}}\right)^{-1} \frac{c_t}{\sigma^{2}} \right)
\end{aligned}
\label{eq:linear bandit posterior}
\end{equation}
where
\begin{equation}
\begin{aligned}
    S_t &= X_t^TX_t\\
    c_t &= X_t^Ty_t
\end{aligned}
\end{equation}
Then final posterior parameters turn out to be
\begin{equation}
\begin{aligned}
    \Lambda_T &= \Lambda_0 + \sum_{t=1}^T \frac{S_t}{\sigma^{2}} - \frac{S_t}{\sigma^{2}} \left(\Sigma^{-1}+ \frac{S_t}{\sigma^{2}}\right)^{-1} \frac{S_t}{\sigma^{2}}\\
    \mu_T &= \Lambda_T^{-1} \left( \Lambda_{0}\mu_{0} + \sum_{t=1}^T \frac{c_t}{\sigma^{2}} - \frac{S_t}{\sigma^{2}} \left(\Sigma^{-1}+ \frac{S_t}{\sigma^{2}}\right)^{-1} \frac{c_t}{\sigma^{2}} \right)
\end{aligned}
\end{equation}
This concludes the proof.


==> Freq_TS.tex <==
\section{Frequentist Setting}
\label{sec:freq}

\blue{Few sents to overview the section...}

\red{Refer to the Algorithm}

\subsection{Known Variance}
\label{sec:freq_known}

\textbf{Setting. } A \emph{multi-armed bandit} \cite{lai85asymptotically,auer02finitetime,lattimore19bandit} is an online learning problem where the learning agent pulls $K$ arms in $n$ rounds. In round $t \in [n]$, the agent pulls arm $I_t \in [K]$ and receives its reward. The reward of arm $i \in [K]$ in round $t$, $Y_{i, t}$, is drawn i.i.d.\ from a distribution of arm $i$, $P_i$, with mean $\mu_i$ and support $[0, 1]$. The means are unknown to the learning agent. The objective of the agent is to maximize its expected cumulative reward in $n$ rounds.

We assume that arm $1$ is optimal, that is $\mu_1 > \max_{i > 1} \mu_i$. Let $\Delta_i = \mu_1 - \mu_i$ be the \emph{gap} of arm $i$, the difference in the expected rewards of arms $1$ and $i$. Then maximization of the expected $n$-round reward can be viewed as minimizing the \emph{expected $n$-round regret}, which we define as
\begin{align}
  R(n)
  = \sum_{i = 2}^K \Delta_i \E{\sum_{t = 1}^n \I{I_t = i}}\,.
  \label{eq:regret_freq}
\end{align}

\subsection{Analysis for General Randomized Exploration \citep{giro}}
\label{sec:gre_analysis}

\citep{giro} proved the following regret upper bound of their algorithm `General Randomized Exploration' (Alg. 1) in a multi-armed bandit with $K$ arms. The distribution $p$ in line \ref{alg:gre:estimate} of \cref{alg:gre} is a function of the history of the arm. For $s \in [n] \cup \set{0}$, let
\begin{align}
  Q_{i, s}(\tau)
  = \condprob{\tilde{\mu}_{i,s} \geq \tau}{\tilde{\mu}_{i,s} \sim p(\cH_{i, s}), \, \cH_{i, s}}
  \label{eq:optimism}
\end{align} \todob{The above is due to my bad notation. $\tilde{\mu}_{i,s} \sim p(\cH_{i, s})$ should be in the subindex.}
be the tail probability that $\tilde{\mu}$ conditioned on history $\cH_{i, s}$ is at least $\tau$ for some tunable parameter $\tau$.

\begin{thm}[\cite{giro}]
\label{thm:gre upper bound} 
For any tunable parameters $(\tau_i)_{i = 2}^K \in \realset^{K - 1}$, the expected $n$-round regret of \cref{alg:gre} can be bounded from above as $R(n) \leq \sum_{i = 2}^K \Delta_i (a_i + b_i)$, where
\begin{align*}
  a_i
  & = \sum_{s = 0}^{n - 1} \E{\min \set{1 / Q_{1, s}(\tau_i) - 1, n}}\,, \\
  b_i
  & = \sum_{s = 0}^{n - 1} \prob{Q_{i, s}(\tau_i) > 1 / n} + 1\,.
\end{align*}
\end{thm}

We now would analyze the bounds for Variance-sensitive Gaussian rewards, where we assume that reward of arm $i$ $\sim \cN(\mu_i,\sigma_i)$.
\begin{cor}[Variance-Aware Regret bounds for Gaussian Rewards]
\label{thm:freq_reg_gauss} 
The expected $n$-round regret of $\giro$ (\red{rename}) is bounded above as:
\[
R(n) \leq \sum_{i = 2}^K \Bign{\frac{62 \sigma_i^2}{\Delta_i} (2\log (n) + 1) + 4\Delta_i}.
\]
\iffalse %%%%%%%%%%%%%
\red{To be updated}...
 For any $a > 1 / \sqrt{2}$, the expected $n$-round regret of $\giro$ is bounded from above as
\begin{align}
  R(n)
  \leq \sum_{i = 2}^K \Delta_i
  \Bigg[& \underbrace{\left(\frac{16 (2 a + 1) c}{\Delta_i^2} \log n + 2\right)}_
  {\text{\emph{Upper bound on $a_i$ in \cref{thm:gre upper bound}}}} + {}
  \label{eq:upper bound} \underbrace{\left(\frac{8 (2 a + 1)}{\Delta_i^2} \log n + 2\right)}_
  {\text{\emph{Upper bound on $b_i$ in \cref{thm:gre upper bound}}}}\Bigg]\,,
  \nonumber
\end{align}
where $b = (2 a + 1) / [a (a + 1)]$ and
\begin{align*}
  c
  = \frac{2 e^2 \sqrt{2 a + 1}}{\sqrt{2 \pi}} \exp\left[\frac{8 b}{2 - b}\right]
  \left(1 + \sqrt{\frac{2 \pi}{4 - 2 b}}\right)
  \nonumber
\end{align*}
is an upper bound on the expected inverse probability of being optimistic, which is derived in \cref{sec:optimism upper bound}.
\fi %%%%%%%%%%%%%%%%%%
\end{cor}

\begin{proof}
\textbf{Algorithmic Notations. } Let $\mu_i \in [0,1]$ be the true mean reward of arm $i$ (with known reward variance $\sigma_i$), for any $i \in [K]$. Assume the algorithm draws the arm according to the posterior samples $\tmu_{i,s} \sim \cN(\hmu_{i,s},\sigma_i)$, 
%
where $\hmu_{i,s}$ being the posterior mean of arm $i$ after the arm is pulled for $s$ times. %We also assume that $\hmu_{i,0} = 0$ and the posterior variance is $\sigma_{i,0} = 1$. %\red{check with BKV}. 
%

\noindent
Given the result of \cref{thm:gre upper bound} our proof has two parts:

\noindent
\textbf{(i) Bounding $b_i$:}

\noindent
Let us assume $\tau_i = \mu_i + \Delta_i/2$. And let us define the event $\cE_{i,s}: = \{\hmu_{i,s} - \mu_i < \Delta_i/4 \}$.

\begin{align*}
\P  (Q_{i,s} & (\tau_i) > 1/n)
	\\
	& =  
	\P(Q_{i,s}(\tau_i) > 1/n \cap \cE_{i,s}) + \P(Q_{i,s}(\tau_i) > 1/n \cap \cE_{i,s}^c)
	\\	
	& \overset{(a)}{\leq} 
	0 + \P(\cE_{i,s}^c) = \P(\hmu_{i,s} - \mu_i \geq \Delta_i/4)
	\leq 
	 1/n
\end{align*} 

where the last inequality follows by \cref{lem:concs} for any $s > \frac{32\sigma_i^2 (\ln n + 1)}{\Delta_i^2}$. Further the inequality $(a)$ follows by noting \[\P\big(Q_{i,s}(\tau_i) > 1/n \cap \cE_{i,s} \big) = 0,
\]
since by \cref{lem:concs}, we can show for any $s > \frac{32 \sigma_i^2 \log n}{\Delta_i^2} $, under the event $\cE_{i,s}$:
\begin{align}
\label{eq:1}
Q_{i,s}(\tau_i)& = \condprob{\tilde{\mu}_{i,s} - \mu_i \geq \Delta_i/2 \cap \hmu_{i,s} - \mu_i < \Delta_i/4}{\tilde{\mu}_{i,s}  \sim p(\cH_{i, s}), \, \cH_{i, s}}  \nonumber\\
& = \P\Bign{(\tmu_{i,s} - \mu_i + \hmu_{i,s} -\hmu_{i,s}) \geq \Delta_i/2 \cap \hmu_{i,s} - \mu_i < \Delta_i/4 \mid \tilde{\mu}_{i,s}  \sim p(\cH_{i, s}), \, \cH_{i, s}} \nonumber
	\\
	& \leq \P(\tmu_{i,s} -\hmu_{i,s} \geq \Delta_i/4)
	\leq 1/n,
\end{align} \todob{The derivation is confusing. Write out $Q_{i,s}(\tau_i)$ and then apply $\cE_{i,s}$.}
where the last inequality follows from the second part of \cref{lem:concs} and since we assumed $s > \frac{32 \sigma_i^2}{\Delta_i^2} \log n$.

\noindent
\textbf{(ii) Bounding $a_i$:} 

\noindent
Let us assume $\tau_i = \mu_i - \Delta_i/2$ and define the event $\cE_{i,s}: = \{\mu_1 - \hmu_{1,s} < \Delta_i/4 \}$. \todob{This is later used as $\cE_{1,s}$.}

We start by noting that $\cE_{i,s} \implies 1 - Q_{1,s}(\tau_i) \leq 1/n$ (i.e. $Q_{1,s}(\tau_i) \geq 1-1/n$). Let us denote the event $\cF_{i,s}:= Q_{1,s}(\tau_i) \geq 1 - 1/n$. The claim follows as when $\cF_{i,s}$ holds, we have: 

\begin{align}
\label{eq:2}
1 - Q_{1,s}(\tau_i)  & = \condprob{\tilde{\mu}_{1,s} - \mu_1 < -\Delta_i/2 \cap \mu_1 -\hmu_{1,s} < \Delta_i/4}{\tilde{\mu}_{1,s}  \sim p(\cH_{1, s}), \, \cH_{1, s}}  \nonumber
\\
& = 
\P\Bign{(\tmu_{1,s} - \mu_1 + \hmu_{1,s} -\hmu_{1,s}) < -\Delta_i/2 \cap \mu_1 -\hmu_{1,s} < \Delta_i/4 \mid \tilde{\mu}_{1,s}  \sim p(\cH_{1, s}), \, \cH_{1, s}} \nonumber
\\
& = 
\P\Bign{(\mu_1 - \tmu_{1,s} + \hmu_{1,s} -\hmu_{1,s}) > \Delta_i/2 \cap \mu_1 -\hmu_{1,s} < \Delta_i/4 \mid \tilde{\mu}_{1,s}  \sim p(\cH_{1, s}), \, \cH_{1, s}} \nonumber\\
& \leq 
\P(\hmu_{1,s} -\tmu_{1,s} \geq \Delta_i/4)
	\leq 1/n^2,
\end{align} 
%\todob{Extra parentheses on the RHS.} 
\todob{The derivation is confusing. Write out $Q_{1,s}(\tau_i)$ and then apply $\cE_{1,s}$.}
where the last inequality follows from the second part of \cref{lem:concs} and since we assumed $s > \frac{64 \sigma_i^2}{\Delta_i^2} \log n$.

Having established this, now we note that for any $s > \frac{32 \sigma_i^2}{\Delta_i^2} (2\log (n) + 1)$: %\todob{Something missing.}:

\begin{align*}
& \E{\min \bigg \{ \frac{1}{Q_{1,s}(\tau_i)}-1,n \bigg \} } 
\\
	& \leq  
	\E{\min\{1/Q_{1,s}(\tau_i)-1,n\}1(\cE_{i,s})} + \E{\min\{1/Q_{1,s}(\tau_i)-1,n\}1(\cE^c_{i,s})}\\
	& \leq
	\E{\min\{\frac{1}{Q_{1,s}(\tau_i)}-1,n\}1(\cE_{i,s})1(\cF_{1,s})} + 
	\E{\min\{\frac{1}{Q_{1,s}(\tau_i)}-1,n\}1(\cE_{i,s})1(\cF^c_{1,s})}	\\
	& \quad\quad\quad\quad\quad\quad\quad\quad
	+ \E{\min\{\frac{1}{Q_{1,s}(\tau_i)}-1,n\}1(\cE^c_{i,s})}\\
	& \leq 
	\frac{1}{n}\E{1(\cE_{1,s})1(\cF_{1,s})} + 
	n\E{1(\cE_{i,s})1(\cF^c_{1,s})}	+ n\E{1(\cE^c_{i,s})}\\
	& \leq 
	\frac{1}{n}\P{(\cE_{i,s} \cap \cF_{1,s})} + 
	n\P{(\cE_{i,s} \cap \cF^c_{1,s})}	+ n\P{(\cE^c_{i,s})}	\\
	& \overset{(a)}{\leq} 
	1/n(1 - 1/n) + n 1/n^2 + n 1/n^2 \leq 3/n,
\end{align*} \todob{I do not understand the need for $\cF_{1,s}$.}
where inequality (a) follows from \cref{eq:2} and \cref{lem:concs} implies $\P(\cE^c_{i,s}) < \frac{1}{n^2}$ for any $s > \frac{32 \sigma_i^2}{\Delta_i^2} (2\log (n) + 1)$. 

Suppose $s_0 = \frac{32 \sigma_i^2}{\Delta_i^2} (2\log (n) + 1)$. The final bound now follows by combining the main regret upper bound of \cref{thm:gre upper bound} (from \cite{giro}) with the above derived upper bounds $a_i$ and $b_i$ as:

\begin{align*}
R(n) & \leq \sum_{i = 2}^K \Delta_i (a_i + b_i)
\\
& \leq 
	\sum_{i = 2}^K \Delta_i \biggn{\sum_{s = 0}^{n - 1} \E{\min \set{1 / Q_{1, s}(\tau_i) - 1, n}} + \sum_{s = 0}^{n - 1} \prob{Q_{i, s}(\tau_i) > 1 / n} + 1}
\\
& \leq
	\sum_{i = 2}^K \Delta_i \biggn{2s_0 + \sum_{s = s_0+1}^{n - 1} \E{\min \set{1 / Q_{1, s}(\tau_i) - 1, n}} + \sum_{s = s_0}^{n - 1} \prob{Q_{i, s}(\tau_i) > 1 / n} + 1}
\\
& \leq 
\sum_{i = 2}^K \Bign{\frac{62 \sigma_i^2}{\Delta_i} (2\log (n) + 1) + 4\Delta_i}
\end{align*}

\red{some problem} - $\tau_i$s are different for $a_i, b_i$ + how to bound $a_i$ for small $s$? \todob{I do not understand the issue.}

\end{proof}


\subsubsection{Concentrations...} 

\todob{We need plain English to explain the reasoning behind the choices of the prior mean and variance.}

\begin{lem}
\label{lem:concs}
For every arm $i \in [K]$ and time step $s \in [T]$, let us define: 

\begin{align*}
\hat \mu_{i,s} = \frac{1}{\sigma_i^{2} + s}\sum_{\ell = 1}^s Y_{i,\ell},
\end{align*}

where $Y_{i,s}$s are iid draws from any $\sigma_i$-subGaussian random variable with mean $\mu_i >0$. Then for any $\epsilon > 0$, 

\begin{align*}
\P(\hmu_{i,s} & -\mu_{i} \geq \epsilon) \leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}}~~ \forall i \in [K]\sm\{1\} \text{ and }\\
& \P(\hmu_{1,s}-\mu_{1} \leq -\epsilon) \leq e \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}} 
\end{align*}

Further for any $i\in [K]$ we always have: 
\begin{align*}
\P(\tmu_{i,s} & -\hmu_{i} \geq \epsilon)
= 
\P(\tmu_{i,s} -\hmu_{i} \leq -\epsilon)
\leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}} 
~~ \forall i \in [K]
\end{align*}

\end{lem}

\begin{proof}
Note we get:

\begin{align*}
\P(\hat \mu_{i,s}  - \mu_i \geq \epsilon)
 & = \P\biggn{\frac{1}{s + \sigma_i^2} \sum_{\ell = 1}^s Y_{i,\ell} - \mu_i \leq \epsilon }\\
 & = \P\biggn{\sum_{\ell = 1}^s Y_{i,\ell} - s\mu_i \geq (s+\sigma_i^2) \epsilon + \sigma_i^2 \mu_i }\\
 & \leq \P\biggn{\sum_{\ell = 1}^s Y_{i,\ell} - s\mu_i \geq s \epsilon } \hfill \text{ since } (\mu_i + \epsilon)\sigma_i^2 > 0\\
 & = \P\biggn{\frac{1}{s}\sum_{\ell = 1}^s Y_{i,\ell} - \mu_i \geq \epsilon } \leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}}, \end{align*}
where the last inequality follows from subGaussian concentration.

On the other hand, 

\begin{align*}
\P(\hat \mu_{1,s}  - \mu_1 \leq -\epsilon) & = \P(\mu_1 - \hat \mu_{1,s}   \geq \epsilon)
 = \P\biggn{\mu_1 - \frac{1}{s + \sigma_1^2} \sum_{\ell = 1}^s Y_{1,\ell}  \geq \epsilon }\\
 & = \P\biggn{s\mu_1 - \sum_{\ell = 1}^s Y_{1,\ell}  \geq (s+\sigma_1^2) \epsilon - \sigma_1^2 \mu_1 }\\
 & = \P\biggn{\mu_1 - \frac{1}{s}\sum_{\ell = 1}^s Y_{1,\ell}  \geq \Big(1+\frac{\sigma_1^2}{s}\Big) \epsilon - \frac{\sigma_1^2 \mu_1}{s} }\\
 & \leq \P\biggn{\sum_{\ell = 1}^s Y_{i,\ell} - s\mu_i \geq s \epsilon } \\
& \overset{(a)}{\leq} \exp\Bign{-\frac{s\biggn{\Big(1+\frac{\sigma_1^2}{s}\Big) \epsilon - \frac{\sigma_1^2 \mu_1}{s}}^2}{2\sigma_i^2}}\\
 %
 & \leq \exp\biggn{-\Bign{\frac{s\epsilon^2}{2\sigma_1^2} - \mu_1\epsilon}} \hfill \text{ since } \frac{\sigma_1^2\mu_1^2}{2s} > 0 ~\forall s\\
 & \leq \exp\biggn{-\Bign{\frac{s\epsilon^2}{2\sigma_1^2} - 1}}  \hfill \text{ since } (\mu_i\epsilon) < 1, \text{ as } \epsilon > 0 \text{ and } \mu_i \in [0,1] \\
 & = e\exp\Bign{-\frac{s\epsilon^2}{2\sigma_1^2}}, 
 \end{align*}
where the inequality (a) again follows from subGaussian concentration. This concludes the first part of the proof.

For the second part, firstly, it is easy to follow that since $\tilde \mu_{i,s} \sim \cN(\hat \mu_{i,s}, \sigma_i^2)$, $\sigma_i$ being the (known) variance of arm $i$, from the subGaussian concentration, we have: 

\begin{align*}
\P \big( & \hat \mu_{i,s} - \tilde \mu_{i,s} \geq \epsilon \big) = \P \big( \hat \mu_{i,s} - \tilde \mu_{i,s} \leq -\epsilon \big)
 \leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}}.
\end{align*}
\end{proof}

\subsection{Unknown Variance}
\label{sec:freq_unknown}

==> bayes_known_arxiv.tex <==
\section{Gaussian Bandit with Known Variances}
\label{sec:bayes_known}

We start with the Bayesian setting with Gaussian rewards and known heterogeneous reward variances. In \cref{sec:bayes_known_algo}, we introduce a Thompson sampling algorithm \citep{thompson33likelihood,chapelle11empirical,agrawal12analysis,russo14learning,gopalan14thompson} for this setting. Gaussian TS is straightforward and appeared in many prior works, starting with \citet{agrawal13further}. We state the regret bound and discuss it in \cref{sec:known_reg}, and sketch its proof in \cref{sec:known_reg_prf}. The regret bound scales roughly as: 
%\todob{Make sure that the parentheses are tall enough for the math inside them. See below. This is at multiple places.} 
%\todob{Do we do colons before display math? Choose one style and stick to it. This is at multiple places.}
\begin{align}
  \textstyle
  \sqrt{n\log n} \sqrt{\sum_{i =1}^K\sigma_i^2
  \log\Big(1 + n\frac{\sigma_{0,i}^{2}}{\sigma_i^{2}}\Big)}\,.
  \label{eq:rough bound known}
\end{align}
One notable property of the bound is that it goes to zero as either the reward variances $\sigma_i^2$ or the prior variances of the mean arm rewards $\sigma_{0, i}^2$ do. Although the bound is novel, its proof mostly follows \citet{kveton21metathompson}. The main reason for stating the bound is to contrast it with the main result in \cref{sec:bayes_unknown2}.

\input{algo_bayes_known.tex}


\subsection{Regret Analysis}
\label{sec:known_reg}

Before we analyze \cref{alg:bayes_known}, we recall the problem setting. The mean arm rewards are sampled from a Gaussian prior, $\bmu \sim P_0 = \cN(\bmu_0, \diag{\bsigma_0^2})$, where $\bmu_0 \in \realset^K$ and $\bsigma_0^2 \in \R_{\geq 0}^K$ are the prior means and variances of $\bmu$, respectively. Both $\bmu_0$ and $\bsigma_0^2$ are known by the agent. The reward of arm $i$ in round $t$ is sampled as $x_{t,i} \sim \cN(\mu_i,\sigma_i^2)$. The reward variances $\bsigma^2$ are fixed and known. Our regret bound is presented below.

\begin{restatable}[Variance-dependent regret bound for known variances]{thm}{bayesknown}
\label{thm:bayes_known} Consider the above setting. Then for any $\delta > 0$, the Bayes regret of Gaussian TS is bounded as:
\begin{align*}
  & R_n
  \leq \sum_{i = 1}^K\sqrt{\frac{2 \sigma_{0,i}^2}{\pi}} n \delta + \sqrt{2n} \sqrt{\sum_{i =1}^K\sigma_i^2\Big(\log(1 + n\sigma_{0,i}^{2}\sigma_i^{-2}) + \sigma_{0,i}^{2}\sigma_i^{-2}\Big)\log(1/\delta)}\,.
\end{align*}
\end{restatable}

\textbf{Discussion.} For $\delta = 1 / n$, the bound in \cref{thm:bayes_known} scales roughly as:
\begin{align*}
  {O}\left(\sqrt{n \log n}\Bigg(\sqrt{\sum_{i = 1}^K\sigma_i^2 \log\Bign{1 + n\sigma_{0,i}^{2}\sigma_i^{-2} } + \sum_{i = 1}^K \sigma_{0,i}^2}\Bigg)\right)\,.
\end{align*} %\todob{This is written in a funny way. We decide to ignore $\log n$ from $\log(1 / \delta)$ because of $\tilde{O}$. But we keep the others. One way out is to present this result similarly to Theorem 2.}
Note here we ignore the first term in \cref{thm:bayes_known}, which is order-wise dominated by the second term when $\delta = 1 / n$. 
% 
Our bound has several properties that we discuss next. First, it matches the usual $\sqrt{n}$ dependence of all classic Bayes regret bounds \citep{russo14learning,russo16information,lu19informationtheoretic}. Second, it increases with variances $\sigma_i^2$ of individual arm rewards, which is expected because higher reward variances make learning harder. Third, the bound can be viewed as a generalization of existing bounds that assume homogeneous reward variance. Specifically, \citet{kveton21metathompson} derive a $\tilde{O}(\sqrt{\sigma^2 K n})$ Bayes regret bound in Lemma 4 under the assumption that the reward distribution of arm $i$ is $\cN(\mu_i, \sigma^2)$. We match it when $\sigma_i = \sigma$ for all arms $i$. Fourth, the bound approaches zero as $\sigma_{0, i} \to 0$. In this setting, the mean arm reward $\mu_i$ is almost certain because its prior variance $\sigma_{0, i}^2$ is low, and no exploration is necessary. This is a unique property of Bayes regret bounds that is not captured by similar frequentist analyses, such as that of \ucbnormal \citep{auer02finitetime}.

We do not provide a matching lower bound and this is a general issue in all recent works on Bayes regret minimization. Starting with seminal works \citep{russo14learning,russo16information}, all Bayes regret bounds are $O(\sqrt{n})$ and no matching lower bounds are derived. The only Bayesian lower bound that we are aware of is $O(\log^2 n)$ for a $K$-armed bandit (Theorem 3 of \citet{lai87adaptive}). In summary, matching Bayes regret upper and lower bounds are an open research problem. Therefore, to validate the shape of our bound, we discuss its behavior in all parameters of interest and relate it to prior regret bounds accepted by the community.


\subsection{Proof Sketch of \cref{thm:bayes_known}}
\label{sec:known_reg_prf}

We sketch the proof of \cref{thm:bayes_known} below. The complete proof can be found in \cref{app:known}.

Let $\bmu_t \in \realset^K$ denote the vector of unknown mean arm rewards at round $t$, sampled as $\mu_{t,i} \sim \cN(\hat\mu_{t,i},\sigma_{t,i}^2)$ for all $i \in [K]$. 
%\todob{$\bmu_{t,i}$ should not be bold.} \todob{Say that $\bmu_t$ are the true unknown mean arm rewards. This is to distinguish it from $\tilde{\bmu}_t$.} 
Let $H_t$ denote the history in round $t$. We also define a high-probability confidence interval for arm $i$ in round $t$ as $C_t(i) = \sqrt{2 \sigma_{t, i}^2 \log(1 / \delta)}$, where $\delta > 0$ is the confidence level, and event:
%
\begin{align*}
  E_t
  = \set{\forall i \in [K]: \abs{\mu_i -  \hat{\mu}_{t,i}} \leq C_t(i)}
\end{align*}
%
that all confidence intervals in round $t$ hold. Now let us fix round $t$. We start by noting that the instantaneous regret at round $t$ can be bounded as:
%
\begin{align*}
  & \E{\mu_{A^*} - \mu_{A_t}}
  = \E{\condE{\mu_{A^*} - \mu_{A_t}}{H_t}} \\
  & = \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}} +
  \E{\condE{{{\hat{\mu}_{t,A_t}}} - \mu_{A_t}}{H_t}}
  \\ & = \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}}\,.
\end{align*} %w\todob{We also need to say that "The second equality holds because $A_t \mid H_t$ and $A^* \mid H_t$ have the same distributions, and $\hat{\mu}_t$ is deterministic given history $H_t$" - \red{this is discussed later}}
%
%The first equality is an application of the tower rule. The second equality holds because $A_t \mid H_t$ and $A^* \mid H_t$ have the same distributions, and $\hat{\mu}_t$ is deterministic given history $H_t$. 
The last equality holds since given $H_t$, clearly $E[\mu_{i}\mid H_t] 
 = \hat{\mu}_{t,i}$ for any $i \in [K]$.
% 
Then we introduce event $E_t$ to deal with the remaining term as:
\begin{align*}
  & \condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}} }{H_t} =  \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar E_t}}{H_t}
  \\
  & \hspace{1.2in}
  + \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{E_t}}{H_t}
  \\
  & \leq \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar{E}_t}}{H_t} + \condE{C_t(A_t)}{H_t}\,,
\end{align*}
where the inequality follows from the observation that
$
  \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{E_t}}{H_t}
  \leq \condE{C_t(A^*)}{H_t}\,,
$
and further $A_t \mid H_t$ and $A^* \mid H_t$ have the same distributions given $H_t$. 
%
Also given history $H_t$, since $\hat{\mu}_t$ is deterministic, $\bmu - \hat{\bmu}_t \mid H_t \sim \cN(\mathbf{0}, \Sigma_t)$, we get:
%\red{above should have the scale factor $b \geq (\mu^* - \mu_i)$?, what is a suitable $b$?}
\begin{align}
\label{eq:thm11}
  & \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar{E}_t}}{H_t} \nonumber
  \\
  & \leq \sum_{i = 1}^K \frac{1}{\sqrt{2 \pi \sigma_{t, i}^2}}
  \int_{x = C_t(i)}^\infty x
  \exp\left[- \frac{x^2}{2 \sigma_{t, i}^2}\right] \dif x
  %\nonumber \\
  %& = \sum_{i = 1}^K - \sqrt{\frac{\sigma_{t, i}^2}{2 \pi}}
  %\int_{x = C_t(i)}^\infty \frac{\partial}{\partial x}
  %\left(\exp\left[- \frac{x^2}{2 \sigma_{t, i}^2}\right]\right) \dif x
  \nonumber \\
  & = \sum_{i = 1}^K \sqrt{\frac{\sigma_{t, i}^2}{2 \pi}} \delta
  \leq \sum_{i = 1}^K \sqrt{\frac{\sigma_{0,i}^2}{2 \pi}}  \delta\,.
\end{align}
%
Having established the above bounds, summing the instantaneous regret over $n$ rounds, the Bayes regret of \cref{alg:bayes_known} can be bounded as:
\begin{align*}
  \E{\sum_{t = 1}^n \mu_{A^*} - \mu_{A_t}}
  \leq \E{\sum_{t = 1}^n C_t(A_t)} +
  \sum_{i = 1}^K\sqrt{\frac{2 \sigma_{0,i}^2}{\pi}} n \delta\,.
\end{align*}
%
The last part is to bound $\E{\sum_{t = 1}^n C_t(A_t)}$ from above. We apply a series of Cauchy-Schwarz inequalities, carefully handle the form of the confidence terms $C_t(i)$, and apply \cref{lem:reciprocal sum}, which yields: %\todob{Two indicators below are written differently from earlier. Choose one notation for indicators and stick to it.}
%
\begin{align*}
  & \E{\sum_{t = 1}^n C_t(A_t)}
  = \E{\sum_{t = 1}^n \sum_{i = 1}^K \I{A_t = i} C_t(i)} 
  \\
  &\leq \E{\sum_{i = 1}^K \bigg[ \sqrt{N_t(i)} \sqrt{\sum_{t = 1}^n C_t^2(i)\I{A_t = i} }\bigg]}
  \\
  & \leq  \sqrt{2n} \sqrt{\sum_{i =1}^K\sigma_i^2\log(1 + n\sigma_{0,i}^{2}\sigma_i^{-2})\log(1/\delta)} + \sqrt{2n\sum_{i = 1}^K\sigma_{0,i}^{2}\log(1/\delta)}
  \,,
\end{align*} 
where recall from \cref{alg:bayes_known} that $N_{t+1}(i) = N_t(i)+\I{A_t=i}$ for all $i \in [K]$ denotes the number of times arm $i$ is pulled in $t$ rounds.
%
%\todob{$N_t(i)$ is not properly quantified.} 
%\todob{A simpler application of Cauchy-Schwarz would be $\sum_{t = 1}^n C_t(A_t) \leq \sqrt{n} \sqrt{\sum_{t = 1}^n C_t^2(A_t)} = \sqrt{n} \sqrt{\sum_{i = 1}^K \sum_{t = 1}^n \I{A_t = i} C_t^2(A_t)}$. Note that there is no need for the expectation. This is all worst case.}
Chaining of all inequalities concludes the proof.

% While this section presents a clean variance-sensitive regret bound for Gaussian bandits (see \cref{thm:bayes_known} and its following discussion), our primary goal is to design a general TS algorithm with variance adaptive regret bounds even when the reward variances are unknown. We present this algorithm next, in \cref{alg:bayes_unknown}, and analyze its regret in \cref{thm:bayes_unknown2}.


==> bayes_unknown_arxiv.tex <==
\section{Gaussian Bandit with Unknown Variances}
\label{sec:bayes_unknown2}

The main contribution of this work is that we consider the Bayesian setting with Gaussian rewards and unknown heterogeneous reward variances. Similarly to \cref{sec:bayes_known}, we propose a Thompson sampling algorithm for this setting in \cref{sec:bayes_unknown_algo}. The algorithm is novel and generalizes even that of \citet{honda14optimality}, which is the closest related work in the frequentist setting. We state the regret bound and discuss it in \cref{sec:unknown_reg}, and sketch its proof in \cref{sec:unknown_reg_prf}. The regret bound scales roughly as:
\begin{align*}
  \textstyle
  \sqrt{n \log n}\sqrt{\sum_{i = 1}^K \frac{\beta_{0,i}}{\alpha_{0,i}-1}
  \log\Big( 1+\frac{n}{\kappa_{0,i}}\Big)}\,,
\end{align*}
where $\frac{\beta_{0, i}}{\alpha_{0, i} - 1}$ represents a proxy for the reward variance $\sigma_i^2$ in \eqref{eq:rough bound known} and $\kappa_{0, i}^{-1}$ plays the role $\sigma_{0, i}^2/\sigma_i^2$. Since the dependencies are analogous, the bound captures the structure of the problem similarly to \eqref{eq:rough bound known}. \emph{The main novelty in the proof is in handling the uncertainty of reward variances $\bsigma^2$, which is very unique among all existing TS proofs.}

\input{algo_bayes_unknown.tex}


\subsection{Regret Analysis}
\label{sec:unknown_reg}

Before we analyze \cref{alg:bayes_unknown}, we recall the problem setting. We assume that the bandit instance $(\bmu, \bsigma)$ is sampled jointly from a Gaussian-Gamma distribution. More specifically, for any arm $i$, the mean and variance of its rewards are sampled as $(\mu_i, \sigma_i^{-2}) \sim NG(\mu_{0, i}, \kappa_{0, i}, \alpha_{0, i}, \beta_{0, i})$, where $(\bmu_0, \bkappa_0, \balpha_0, \bbeta_0)$ are known prior parameters. This can also be seen as first sampling $\sigma_i^{-2} \sim \text{Gam}(\alpha_{0,i},\beta_{0,i})$ and then $\mu_i \sim \cN(\mu_{0,i}, \frac{\sigma_i^2}{\kappa_{0,i}})$. Our regret bound is presented below.

\begin{restatable}[Variance-dependent regret bound for unknown variances]{thm}{bayesunknown}
\label{thm:bayes_unknown2} Consider the above setting and assume that  $\alpha_{0,i }\geq 1$ for all arms $i \in [K]$. Then for any $\delta > 0$, the Bayes regret of \varts is bounded as:
\begin{align*}
  R_n
  \leq C\sqrt{n \log(1 / \delta)} + \delta C \sqrt{\frac{nK}{2\pi}}\,,
\end{align*}
where $C^2 = \sum_{i = 1}^K \frac{\beta_{0,i}}{\alpha_{0,i} - 1} \biggn{ \frac{2}{\kappa_{0,i}} + \frac{0.5}{\kappa_{0,i}(\alpha_{0,i}-1)} + 5\log\Big(1 + \frac{n}{\kappa_{0,i}}\Big) }$ is a constant dependent on prior parameters.
\end{restatable}

\textbf{Discussion.} For $\delta = 1 / n$, the bound in \cref{thm:bayes_unknown2} is $\tilde{O}(\sqrt{C n})$. The dependence on $\sqrt{n}$ is the same as in \cref{thm:bayes_known}. A closer examination of $C$ reveals many similarities.

First, $\beta_{0, i} / (\alpha_{0, i} - 1)$ is the mean of an Inverse-Gamma distribution with parameters $(\alpha_{0, i}, \beta_{0, i})$. Since $\lambda_i$, the precision of the reward distribution of arm $i$, is sampled from $\text{Gam}(\alpha_{0, i}, \beta_{0, i})$, we have that $\beta_{0, i} / (\alpha_{0, i} - 1)$ is the mean of the variance distribution of arm $i$. That is, $\beta_{0, i} / (\alpha_{0, i} - 1)$ in \cref{thm:bayes_unknown2} plays the role of $\sigma_i^2$ in \cref{thm:bayes_known}.

Second, $\kappa_{0, i}$ in the Gaussian-Gamma prior in the unknown variance case plays the role of $\sigma_i^2 / \sigma_{0, i}^2$ in the known variance case \citep{murphy2007conjugate}. Therefore, as $\kappa_{0, i} \to \infty$, we would expect the bound in \cref{thm:bayes_unknown2} to approach zero, similarly to \cref{thm:bayes_known}. This is clear upon inspecting $C$.

Finally, take $\alpha_{0, i}, \beta_{0, i} \to \infty$ while $\beta_{0, i} / (\alpha_{0, i} - 1)$ is kept constant. In this setting, the term $0.5 / (\kappa_{0, i} (\alpha_{0, i} - 1))$ vanishes and we recover the same algebraic form as in \cref{thm:bayes_known}. Therefore, $0.5 / (\kappa_{0, i} (\alpha_{0, i} - 1))$ can be viewed as the cost for not knowing the variance $\sigma_i^2$. In addition, the variance of the Inverse-Gamma distribution of $\sigma_i^2$ approaches zero because it is $O(\beta_{0, i}^2 \alpha_{0, i}^{-3})$. Therefore, our setting approaches that of the known variance, and so does our bound, up to a small multiplicative factor of $5$.

In summary, the known variance bound in \cref{thm:bayes_known} is closely related to the unknown variance bound in \cref{thm:bayes_unknown2}. The additive penalty for not knowing the variance mimics the frequentist setting \citep{audibert09exploration}, although the specific penalty, $0.5 / (\kappa_{0, i} (\alpha_{0, i} - 1))$, differs.


\subsection{Proof Sketch of \cref{thm:bayes_unknown2}}
\label{sec:unknown_reg_prf}

We sketch the proof of \cref{thm:bayes_unknown2} below. The complete proof can be found in \cref{app:unknown}.

The overall structure of the proof is inspired by the analysis of the known variance case (\cref{sec:known_reg_prf}). However, this proof is significantly more involved due to the unknown reward variance and maintaining Gaussian-Gamma posteriors. As in the proof of \cref{thm:bayes_known}, we can decompose the regret in round $t$ as:
\begin{align}
\label{eq:term55}
  & \E{\mu_{A^*} - \mu_{A_t}}
  = \E{\condE{\mu_{A^*} - \mu_{A_t}}{H_t}} = \nonumber \\
  & 
  \hspace{-3pt}
  \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}} +
  \mathbb E\Bigsn{\mathbb E_{\bsigma}\bigsn{\mathbb E [\hat{\mu}_{t,A_t}- \mu_{A_t} \mid \bsigma ] \mid H_t} }\nonumber
  \\
  & = \E{\condE{\mu_{A^*} - {\hat{\mu}_{t,A^*}}}{H_t}} 
\end{align}
where $\sigma_{t,i}^2= \frac{1}{{\kappa_{t,i}\lambda_{t,i}}}$ %\todob{There is no $\sigma_{t, i}^2$ above.} 
is a sampled posterior variance and $\lambda_{t,i} \sim \text{Gam}(\alpha_{t,i},\beta_{t,i})$. 
%\todob{We need to have clearer terminology (also in the algorithm). $\lambda_{t, i}^{-2}$ is the posterior sampled variance of rewards. $\sigma_{t,i}^2$ is the posterior variance of the mean reward.} 
The last equality holds since given $H_t$ and $\bsigma$,  $E[\mu_{i} \mid H_t] = \hat{\mu}_{t,i}$ for any $i \in [K]$ by definition of the posterior update.

Now given $H_t$ and $\bsigma_t$, let us define the high-probability confidence interval of each arm $i$ as $C_t(i) = \sqrt{2 \sigma_{t, i}^2 \log(1 / \delta)}$, and the ``good event"
$
  E_t
  = \set{\forall i \in [K]: \abs{\mu_i -  \hat{\mu}_{t,i}} \leq C_t(i)}
$,
same as what we introduced in the proof of \cref{thm:bayes_known}. 
%\todob{Refer to earlier defined concepts instead of redefining them, especially if you want to make a point that this proof is built on another one.}
%which essentially indicates the ``good event"' %\todob{Use \say{this} for quotes.} when all the confidence intervals at round $t$ hold good. 
%
Further note, given $H_t$ and $\sigma_{t,i}^2$ (or equivalently $\lambda_{t,i})$),  $\mu_i - \hat{\mu}_{t,i} \mid \sigma_{t,i}^2, H_t \sim \cN(\mathbf{0}, \sigma_{t,i}^2)$, 
since given $H_t$ and $\sigma_t$, $\mu_i$ has the posterior $\mu_i \sim \cN(\hat \mu_{t,i}, \sigma_{t,i}^{2})$, where recall we defined $\sigma_{t,i}^2 = \frac{1}{\kappa_{t,i}\lambda_{t,i}}$ and $\lambda_{t,i} = \frac{1}{\sigma_{t,i}^2} \sim \text{Gam}(\alpha_{t,i},\beta_{t,i})$.
 %\red{I am confused a bit}
Thus following same analysis as in \eqref{eq:thm11}, we get: 
%So we w.h.p. $(1-\delta')$, we have \red{checK!}:
%
\begin{align}
  \condE{(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar{E}_t}}{\bsigma_t, H_t}
  \leq \sum_{i = 1}^K \sqrt{\frac{\sigma_{t,i}^2}{2 \pi}} \delta.
  \label{eq:bayes_regret_scale22}
\end{align} %\todob{This seems incorrect. $\sigma_i^2$ should be $\sigma_{t, i}^2$?}
%
Further taking expectation over $H_n, \bsigma, \bmu$, and summing over all $t$ we get:
\begin{align}
\label{eq:long22}
  &\E{\sum_{t = 1}^n(\mu_{A^*} - {\hat{\mu}_{t,A^*}}) \I{\bar{E}_t}}
  \leq 
  \delta(2\pi)^{-1/2}\mathbb{E}_{H_n, \bsigma, \bmu}\biggsn{\sum_{t = 1}^n \sum_{i = 1}^K \mathbb{E}_{\bsigma_{t}}[\sigma_{t,i} \mid \bmu,\bsigma, H_t]}
\end{align}
%
Now one of the main novelty of this proof lies in showing:
\begin{align*}
& \mathbb{E}_{H_n, \bsigma, \bmu}\biggsn{\sum_{t = 1}^n \sum_{i = 1}^K \mathbb{E}_{\bsigma_{t}}[\sigma_{t,i} \mid \bmu,\bsigma, H_t]}
\leq 
\sqrt{nK} \sqrt{\sum_{i = 1}^K \frac{4 \beta_{0,i} + \frac{\beta_{0,i}}{\alpha_{0,i}-1}}{2\kappa_{0,i}(\alpha_{0,1}-1)}
+ 
\sum_{i = 1}^K \frac{5\beta_{0,i}}{(\alpha_{0,i}-1)}\log\Big(1 + \frac{n}{\kappa_{0,i}}\Big)}
\end{align*} 
%\todob{$H_n$ in the inner expectation should be $H_t$. We should not condition on the future.} 
%\todob{Why conditioning on $\bmu$? - \red{used later in the detailed proof, note $\sigma_{t,i}$ depends on $\mu$, etc.}} 
which involves a series of careful applications of tower rule of expectations and \cref{lem:reciprocal sum} (in \cref{app:unknown}) -- this is the most novel part of this proof which shows an elegant way to upper bound $\E{\sigma_{t, i}}$ for any $i$ and $t$. While the analysis is non-trivial and lengthy, the complete proof can be found in \cref{app:unknown}.
%
Now coming back to the original Bayesian regret expression, note that the regret expression from \eqref{eq:term5} 
%\todob{A forward reference to Appendix. Fix if it as an error or say "in Appendix" - \red{I wrote its in Appendix B? Not sure of the issue}} 
can be actually decomposed based on $E_t$ and $\bar E_t$ as:
\begin{align}
\label{eq:term22}
  \condE{{\hat{\mu}_{t,A^*}}  - \mu_{A^*}}{H_t} 
  & \leq \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{E_t}}{H_t} 
  +
  \condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar{E}_t}}{H_t} \nonumber
  \\
  & \leq \condE{C_t(A^*)}{H_t} \nonumber
  +\condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar{E}_t}}{H_t}
  \\
  & = \condE{C_t(A_t)}{H_t} 
  +\condE{({\hat{\mu}_{t,A^*}} - \mu_{A^*}) \I{\bar{E}_t}}{H_t},
\end{align}
where the last equality follows from the fact that $A_t \mid H_t$ and $A^* \mid H_t$ have the same distributions, as both $\tilde \mu_{t,i}$ and $\mu_{t,i}$ can be seen as independent posterior samples from a NG$(\hat \mu_{t,i},\kappa_{t,i},\alpha_{t,i},\beta_{t,i})$.% distribution marginalized over $\lambda$. %\todob{It is unclear what "marginalized over $\lambda$" means here.}

\iffalse%%%%%%%%%%%%%%%%%%
More precisely for any realization of $\tilde \mu_{t,i}$ and $\mu_i$:
\[
P(\tilde \mu_{t,i}) = \int_{\lambda} P\big( (\tilde \mu_{t,i}, \lambda_{t,i} \sim \text{NG}(\hat \mu_{t,i},\kappa_{t,i},\alpha_{t,i},\beta_{t,i}) ) \big)d\lambda  ~~~\text{and}
\]
\[
P(\mu_{i}) = \int_{\lambda} P\big( (\tilde \mu_{t,i}, \lambda_{t,i} \sim \text{NG}(\hat \mu_{t,i},\kappa_{t,i},\alpha_{t,i},\beta_{t,i}) ) \big)d\lambda,
\]
they follow the same distribution. 
\fi%%%%%%%%%%%%%%%%%%%%%%%

The second term in \eqref{eq:term22} is bounded similarly to \eqref{eq:long22}. 
%
The only remaining task is to bound the first term in \eqref{eq:term22}, which again involves some non-trivial chain of inequalities involving tower rule of expectations, Cauchy-Schwarz, Jensen's and \cref{lem:reciprocal root sum}, detailed in \cref{app:unknown}. As a result, the final expression can be bounded as:% \todob{Indicators below are written differently from earlier. Choose one notation for indicators and stick to it.}
%
\begin{align*}
  &\E{\sum_{t = 1}^n C_t(A_t)}
  \\
  &\overset{}{\leq} \E{ \bigg[ \sqrt{\sum_{i = 1}^K N_n(i)} \sqrt{\sum_{i = 1}^K \sum_{t = 1}^n C_t^2(i)\I{A_t = i} }\bigg]}
  \\
  &\overset{}{=}  \bigg[ \sqrt{n} \sqrt{\E{ \sum_{i = 1}^K \sum_{t = 1}^n {2 \sigma_{t, i}^2 \log(1 / \delta)}\I{A_t = i} }\bigg]}
  \\
  &\overset{}{=}  \bigg[ \sqrt{n} \sqrt{\E{ \sum_{i = 1}^K \sum_{s = 0}^{N_n(i)} \bign{2 \sigma_{t, i}^2 \log(1 / \delta)}\I{A_t = i} }\bigg]}
  \\
  & \leq \sqrt{n\log \frac{1}{\delta}} \sqrt{\sum_{i = 1}^K \sum_{i = 1}^K \frac{4 \beta_{0,i} + \frac{\beta_{0,i}}{\alpha_{0,i}-1}}{2\kappa_{0,i}(\alpha_{0,1}-1)}
+ 
\sum_{i = 1}^K \frac{5\beta_{0,i}}{(\alpha_{0,i}-1)}\log\Big(1 + \frac{n}{\kappa_{0,i}}\Big)}
 \,.
\end{align*}
Finally, chaining of the above inequalities on the summation of the instantaneous regret over $n$ rounds, from \eqref{eq:term22} we get:
%\todob{Why the reference to \eqref{eq:term22}?}
%
\begin{align*}
%\label{eq:term2}
  &\mathbb{E}_{H_n,\bmu,\bsigma}\biggsn{\sum_{t = 1}^n\condE{{\hat{\mu}_{t,A^*}}  - \mu_{A^*}}{H_t}} \nonumber
  \leq
  C \biggn{\frac{\delta \sqrt{nK}}{\sqrt{2\pi}} + \sqrt{n\log \frac{1}{\delta}}}
  \,,
\end{align*}
which proves the claim.

%\todob{The structure of the current proof is not good because the connection to the known variance proof seems weak. I would do the following:

%1) Start with (4).

%2) Apply (7).

%3) Bound the second term in (7) using (5). Leave $\sigma_{t, i}^2$ the way it is.

%4) Bound the first term in (7). Tie it to how we bound an analogous term in Theorem 1.

%5) Massage the final bound to get $\E{\sigma_{t, i}^2}$. Finally, apply the main trick, that $\E{\sigma_{t, i}^2}$ has a nice upper bound for any $i$ and $t$. - \red{done!}}

% noting $C:= \sum_{i = 1}^K \frac{4 \beta_{0,i} + \frac{\beta_{0,i}}{\alpha_{0,i}-1}}{2\kappa_{0,i}(\alpha_{0,1}-1)}
%+ 
%\sum_{i = 1}^K \frac{5\beta_{0,i}}{(\alpha_{0,i}-1)}\log\Big(1 + \frac{n}{\kappa_{0,i}}\Big)$. 

% %As described in \cref{rem:unknown}, \cref{thm:bayes_unknown2} gives the first variance-sensitive regret bounds with TS, even for the case of unknown arm variances. 
% We also performed empirical studies to evaluate the efficacy
% of \cref{alg:bayes_unknown}. As reported in the next section, \varts\, significantly overperforms the existing baselines, \ucb \citep{auer02finitetime}, \ucbtuned \citep{auer02finitetime} and \ucbv \citep{audibert09exploration} even in the misspecified setting (i.e. when arm rewards $\bmu$ are not necessarily Gaussian). %, which seconds the practicality of our proposed algorithm, beyond its theoretical regret bounds. 
% \todob{I do not understand this discussion. Simply say that experiments come next. We can summarize the experimental results at the beginning of the experimental section if you want to. - \red{shortened, done!}}


==> freq_known.tex <==
\section{Frequentist Setting}
\label{sec:freq}

\blue{Few sents to overview the section...}

\red{Refer to the Algorithm}

\subsection{Known Variance}
\label{sec:freq_known}

\textbf{Setting. } A \emph{multi-armed bandit} \cite{lai85asymptotically,auer02finitetime,lattimore19bandit} is an online learning problem where the learning agent pulls $K$ arms in $n$ rounds. In round $t \in [n]$, the agent pulls arm $I_t \in [K]$ and receives its reward. The reward of arm $i \in [K]$ in round $t$, $Y_{i, t}$, is drawn i.i.d.\ from a distribution of arm $i$, $P_i$, with mean $\mu_i$ and support $[0, 1]$. The means are unknown to the learning agent. The objective of the agent is to maximize its expected cumulative reward in $n$ rounds.

We assume that arm $1$ is optimal, that is $\mu_1 > \max_{i > 1} \mu_i$. Let $\Delta_i = \mu_1 - \mu_i$ be the \emph{gap} of arm $i$, the difference in the expected rewards of arms $1$ and $i$. Then maximization of the expected $n$-round reward can be viewed as minimizing the \emph{expected $n$-round regret}, which we define as
\begin{align}
  R(n)
  = \sum_{i = 2}^K \Delta_i \E{\sum_{t = 1}^n \I{I_t = i}}\,.
  \label{eq:regret_freq}
\end{align}

\subsection*{Regret Analysis}
\label{sec:freq_known_analysis}

\citep{giro} proved the following regret upper bound of their algorithm `General Randomized Exploration' (Alg. 1) in a multi-armed bandit with $K$ arms. The distribution $p$ in line \ref{alg:gre:estimate} of \cref{alg:gre} is a function of the history of the arm. For $s \in [n] \cup \set{0}$, let
\begin{align}
  Q_{i, s}(\tau)
  = \condprob{\tilde{\mu}_{i,s} \geq \tau}{\cH_{i, s}}
  \label{eq:optimism}
\end{align} 
be the tail probability that $\tilde{\mu}$ conditioned on history $\cH_{i, s}$ is at least $\tau$ for some tunable parameter $\tau$.

\begin{thm}[\cite{giro}]
\label{thm:gre upper bound} 
For any tunable parameters $(\tau_i)_{i = 2}^K \in \realset^{K - 1}$, the expected $n$-round regret of \cref{alg:gre} can be bounded from above as $R(n) \leq \sum_{i = 2}^K \Delta_i (a_i + b_i)$, where
\begin{align*}
  a_i
  & = \sum_{s = 0}^{n - 1} \E{\min \set{1 / Q_{1, s}(\tau_i) - 1, n}}\,, \\
  b_i
  & = \sum_{s = 0}^{n - 1} \prob{Q_{i, s}(\tau_i) > 1 / n} + 1\,.
\end{align*}
\end{thm}

\begin{restatable}[Variance Adaptive Frequentist Regret for Known Variance]{thm}{freqknown}
\label{thm:freq_known}
%\red{Incomplete, don't read this}
Let $\bmu$ be the expected reward vector of the $K$-armed MAB with their respective sub-Gaussianity parameter vector $\bsigma^2$. Then assuming $A_*$ being the optimal arm under $\bmu$ and $A_t$ be the pulled arm in round $t$, the expected $n$-round regret of TS is bounded above as:
\[
\E{\sum_{t = 1}^n \mu(A_*) - \mu(A_t)} \leq \sum_{i = 2}^K \Bign{\frac{62 \sigma_i^2}{\Delta_i} (2\log (n) + 1) + 4\Delta_i}.
\]
\iffalse %%%%%%%%%%%%%
\red{To be updated}...
 For any $a > 1 / \sqrt{2}$, the expected $n$-round regret of $\giro$ is bounded from above as
\begin{align}
  R(n)
  \leq \sum_{i = 2}^K \Delta_i
  \Bigg[& \underbrace{\left(\frac{16 (2 a + 1) c}{\Delta_i^2} \log n + 2\right)}_
  {\text{\emph{Upper bound on $a_i$ in \cref{thm:gre upper bound}}}} + {}
  \label{eq:upper bound} \underbrace{\left(\frac{8 (2 a + 1)}{\Delta_i^2} \log n + 2\right)}_
  {\text{\emph{Upper bound on $b_i$ in \cref{thm:gre upper bound}}}}\Bigg]\,,
  \nonumber
\end{align}
where $b = (2 a + 1) / [a (a + 1)]$ and
\begin{align*}
  c
  = \frac{2 e^2 \sqrt{2 a + 1}}{\sqrt{2 \pi}} \exp\left[\frac{8 b}{2 - b}\right]
  \left(1 + \sqrt{\frac{2 \pi}{4 - 2 b}}\right)
  \nonumber
\end{align*}
is an upper bound on the expected inverse probability of being optimistic, which is derived in \cref{sec:optimism upper bound}.
\fi %%%%%%%%%%%%%%%%%%
\end{restatable}

\begin{proof}
\textbf{Algorithmic Notations. } Let $\mu_i \in [0,1]$ be the true mean reward of arm $i$ (with known reward variance $\sigma_i$), for any $i \in [K]$. Assume the algorithm draws the arm according to the posterior samples $\tmu_{i,s} \sim \cN(\hmu_{i,s},\sigma_i)$, 
%
where $\hmu_{i,s}$ being the posterior mean of arm $i$ after the arm is pulled for $s$ times. %We also assume that $\hmu_{i,0} = 0$ and the posterior variance is $\sigma_{i,0} = 1$. %\red{check with BKV}. 
%

\noindent
Given the result of \cref{thm:gre upper bound} our proof has two parts:

\noindent
\textbf{(i) Bounding $b_i$:}

\noindent
Let us assume $\tau_i = \mu_i + \Delta_i/2$. And let us define the event $\cE_{i,s}: = \{\hmu_{i,s} - \mu_i < \Delta_i/4 \}$.

\begin{align*}
\P  (Q_{i,s} & (\tau_i) > 1/n)
	\\
	& =  
	\P(Q_{i,s}(\tau_i) > 1/n \cap \cE_{i,s}) + \P(Q_{i,s}(\tau_i) > 1/n \cap \cE_{i,s}^c)
	\\	
	& \overset{(a)}{\leq} 
	0 + \P(\cE_{i,s}^c) = \P(\hmu_{i,s} - \mu_i \geq \Delta_i/4)
	\leq 
	 1/n
\end{align*} 

where the last inequality follows by \cref{lem:concs} for any $s > \frac{32\sigma_i^2 (\ln n + 1)}{\Delta_i^2}$. Further the inequality $(a)$ follows by noting \[\P\big(Q_{i,s}(\tau_i) > 1/n \cap \cE_{i,s} \big) = 0,
\]
since by \cref{lem:concs}, we can show for any $s > \frac{32 \sigma_i^2 \log n}{\Delta_i^2} $, under the event $\cE_{i,s}$:
\begin{align}
\label{eq:1}
Q_{i,s}(\tau_i)& = \condprob{\tilde{\mu}_{i,s} - \mu_i \geq \Delta_i/2 \cap \hmu_{i,s} - \mu_i < \Delta_i/4}{\cH_{i, s}}  \nonumber\\
& = \P\Bign{(\tmu_{i,s} - \mu_i + \hmu_{i,s} -\hmu_{i,s}) \geq \Delta_i/2 \cap \hmu_{i,s} - \mu_i < \Delta_i/4 \mid \cH_{i, s}} \nonumber
	\\
	& \leq \P(\tmu_{i,s} -\hmu_{i,s} \geq \Delta_i/4)
	\leq 1/n,
\end{align} \todob{The derivation is confusing. Write out $Q_{i,s}(\tau_i)$ and then apply $\cE_{i,s}$.}
where the last inequality follows from the second part of \cref{lem:concs} and since we assumed $s > \frac{32 \sigma_i^2}{\Delta_i^2} \log n$.

\noindent
\textbf{(ii) Bounding $a_i$:} 

\noindent
Let us assume $\tau_i = \mu_i - \Delta_i/2$ and define the event $\cE_{i,s}: = \{\mu_1 - \hmu_{1,s} < \Delta_i/4 \}$. %\todob{This is later used as $\cE_{1,s}$.}

We start by noting that $\cE_{i,s} \implies 1 - Q_{1,s}(\tau_i) \leq 1/n$ (i.e. $Q_{1,s}(\tau_i) \geq 1-1/n$). Let us denote the event $\cF_{i,s}:= Q_{1,s}(\tau_i) \geq 1 - 1/n$. The claim follows as when $\cF_{i,s}$ holds, we have: 

\begin{align}
\label{eq:2}
1 - Q_{1,s}(\tau_i)  & = \condprob{\tilde{\mu}_{1,s} - \mu_1 < -\Delta_i/2 \cap \mu_1 -\hmu_{1,s} < \Delta_i/4}{\cH_{1, s}}  \nonumber
\\
& = 
\P\Bign{(\tmu_{1,s} - \mu_1 + \hmu_{1,s} -\hmu_{1,s}) < -\Delta_i/2 \cap \mu_1 -\hmu_{1,s} < \Delta_i/4 \mid \cH_{1, s}} \nonumber
\\
& = 
\P\Bign{(\mu_1 - \tmu_{1,s} + \hmu_{1,s} -\hmu_{1,s}) > \Delta_i/2 \cap \mu_1 -\hmu_{1,s} < \Delta_i/4 \mid \cH_{1, s}} \nonumber\\
& \leq 
\P(\hmu_{1,s} -\tmu_{1,s} \geq \Delta_i/4)
	\leq 1/n^2,
\end{align} 
%\todob{Extra parentheses on the RHS.} 
\todob{The derivation is confusing. Write out $Q_{1,s}(\tau_i)$ and then apply $\cE_{1,s}$.}
where the last inequality follows from the second part of \cref{lem:concs} and since we assumed $s > \frac{64 \sigma_i^2}{\Delta_i^2} \log n$.

Having established this, now we note that for any $s > \frac{32 \sigma_i^2}{\Delta_i^2} (2\log (n) + 1)$: %\todob{Something missing.}:

\begin{align*}
& \E{\min \bigg \{ \frac{1}{Q_{1,s}(\tau_i)}-1,n \bigg \} } 
\\
	& \leq  
	\E{\min\{1/Q_{1,s}(\tau_i)-1,n\}1(\cE_{i,s})} + \E{\min\{1/Q_{1,s}(\tau_i)-1,n\}1(\cE^c_{i,s})}\\
	& \leq
	\E{\min\{\frac{1}{Q_{1,s}(\tau_i)}-1,n\}1(\cE_{i,s})1(\cF_{1,s})} + 
	\E{\min\{\frac{1}{Q_{1,s}(\tau_i)}-1,n\}1(\cE_{i,s})1(\cF^c_{1,s})}	\\
	& \quad\quad\quad\quad\quad\quad\quad\quad
	+ \E{\min\{\frac{1}{Q_{1,s}(\tau_i)}-1,n\}1(\cE^c_{i,s})}\\
	& \leq 
	\frac{1}{n}\E{1(\cE_{1,s})1(\cF_{1,s})} + 
	n\E{1(\cE_{i,s})1(\cF^c_{1,s})}	+ n\E{1(\cE^c_{i,s})}\\
	& \leq 
	\frac{1}{n}\P{(\cE_{i,s} \cap \cF_{1,s})} + 
	n\P{(\cE_{i,s} \cap \cF^c_{1,s})}	+ n\P{(\cE^c_{i,s})}	\\
	& \overset{(a)}{\leq} 
	1/n(1 - 1/n) + n 1/n^2 + n 1/n^2 \leq 3/n,
\end{align*} \todob{I do not understand the need for $\cF_{1,s}$.}
where inequality (a) follows from \cref{eq:2} and \cref{lem:concs} implies $\P(\cE^c_{i,s}) < \frac{1}{n^2}$ for any $s > \frac{32 \sigma_i^2}{\Delta_i^2} (2\log (n) + 1)$. 

Suppose $s_0 = \frac{32 \sigma_i^2}{\Delta_i^2} (2\log (n) + 1)$. The final bound now follows by combining the main regret upper bound of \cref{thm:gre upper bound} (from \cite{giro}) with the above derived upper bounds $a_i$ and $b_i$ as:

\begin{align*}
R(n) & \leq \sum_{i = 2}^K \Delta_i (a_i + b_i)
\\
& \leq 
	\sum_{i = 2}^K \Delta_i \biggn{\sum_{s = 0}^{n - 1} \E{\min \set{1 / Q_{1, s}(\tau_i) - 1, n}} + \sum_{s = 0}^{n - 1} \prob{Q_{i, s}(\tau_i) > 1 / n} + 1}
\\
& \leq
	\sum_{i = 2}^K \Delta_i \biggn{2s_0 + \sum_{s = s_0+1}^{n - 1} \E{\min \set{1 / Q_{1, s}(\tau_i) - 1, n}} + \sum_{s = s_0}^{n - 1} \prob{Q_{i, s}(\tau_i) > 1 / n} + 1}
\\
& \leq 
\sum_{i = 2}^K \Bign{\frac{62 \sigma_i^2}{\Delta_i} (2\log (n) + 1) + 4\Delta_i}
\end{align*}

\red{some problem, needs discussion} - $\tau_i$s are different for $a_i, b_i$ + how to bound $a_i$ for small $s$? \todob{I do not understand the issue.}

\end{proof}


\subsubsection{Concentration Results used in the Proof of \cref{thm:freq_known}} 

\todob{We need plain English to explain the reasoning behind the choices of the prior mean and variance.}

\begin{lem}
\label{lem:concs}
For every arm $i \in [K]$ and time step $s \in [T]$, let us define: 

\begin{align*}
\hat \mu_{i,s} = \frac{1}{\sigma_i^{2} + s}\sum_{\ell = 1}^s Y_{i,\ell},
\end{align*}

where $Y_{i,s}$s are iid draws from any $\sigma_i$-subGaussian random variable with mean $\mu_i >0$. Then for any $\epsilon > 0$, 

\begin{align*}
\P(\hmu_{i,s} & -\mu_{i} \geq \epsilon) \leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}}~~ \forall i \in [K]\sm\{1\} \text{ and }\\
& \P(\hmu_{1,s}-\mu_{1} \leq -\epsilon) \leq e \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}} 
\end{align*}

Further for any $i\in [K]$ we always have: 
\begin{align*}
\P(\tmu_{i,s} & -\hmu_{i} \geq \epsilon)
= 
\P(\tmu_{i,s} -\hmu_{i} \leq -\epsilon)
\leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}} 
~~ \forall i \in [K]
\end{align*}

\end{lem}

\begin{proof}
Note we get:

\begin{align*}
\P(\hat \mu_{i,s}  - \mu_i \geq \epsilon)
 & = \P\biggn{\frac{1}{s + \sigma_i^2} \sum_{\ell = 1}^s Y_{i,\ell} - \mu_i \leq \epsilon }\\
 & = \P\biggn{\sum_{\ell = 1}^s Y_{i,\ell} - s\mu_i \geq (s+\sigma_i^2) \epsilon + \sigma_i^2 \mu_i }\\
 & \leq \P\biggn{\sum_{\ell = 1}^s Y_{i,\ell} - s\mu_i \geq s \epsilon } \hfill \text{ since } (\mu_i + \epsilon)\sigma_i^2 > 0\\
 & = \P\biggn{\frac{1}{s}\sum_{\ell = 1}^s Y_{i,\ell} - \mu_i \geq \epsilon } \leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}}, \end{align*}
where the last inequality follows from subGaussian concentration.

On the other hand, 

\begin{align*}
\P(\hat \mu_{1,s}  - \mu_1 \leq -\epsilon) & = \P(\mu_1 - \hat \mu_{1,s}   \geq \epsilon)
 = \P\biggn{\mu_1 - \frac{1}{s + \sigma_1^2} \sum_{\ell = 1}^s Y_{1,\ell}  \geq \epsilon }\\
 & = \P\biggn{s\mu_1 - \sum_{\ell = 1}^s Y_{1,\ell}  \geq (s+\sigma_1^2) \epsilon - \sigma_1^2 \mu_1 }\\
 & = \P\biggn{\mu_1 - \frac{1}{s}\sum_{\ell = 1}^s Y_{1,\ell}  \geq \Big(1+\frac{\sigma_1^2}{s}\Big) \epsilon - \frac{\sigma_1^2 \mu_1}{s} }\\
 & \leq \P\biggn{\sum_{\ell = 1}^s Y_{i,\ell} - s\mu_i \geq s \epsilon } \\
& \overset{(a)}{\leq} \exp\Bign{-\frac{s\biggn{\Big(1+\frac{\sigma_1^2}{s}\Big) \epsilon - \frac{\sigma_1^2 \mu_1}{s}}^2}{2\sigma_i^2}}\\
 %
 & \leq \exp\biggn{-\Bign{\frac{s\epsilon^2}{2\sigma_1^2} - \mu_1\epsilon}} \hfill \text{ since } \frac{\sigma_1^2\mu_1^2}{2s} > 0 ~\forall s\\
 & \leq \exp\biggn{-\Bign{\frac{s\epsilon^2}{2\sigma_1^2} - 1}}  \hfill \text{ since } (\mu_i\epsilon) < 1, \text{ as } \epsilon > 0 \text{ and } \mu_i \in [0,1] \\
 & = e\exp\Bign{-\frac{s\epsilon^2}{2\sigma_1^2}}, 
 \end{align*}
where the inequality (a) again follows from subGaussian concentration. This concludes the first part of the proof.

For the second part, firstly, it is easy to follow that since $\tilde \mu_{i,s} \sim \cN(\hat \mu_{i,s}, \sigma_i^2)$, $\sigma_i$ being the (known) variance of arm $i$, from the subGaussian concentration, we have: 

\begin{align*}
\P \big( & \hat \mu_{i,s} - \tilde \mu_{i,s} \geq \epsilon \big) = \P \big( \hat \mu_{i,s} - \tilde \mu_{i,s} \leq -\epsilon \big)
 \leq \exp\Bign{-\frac{s\epsilon^2}{2\sigma_i^2}}.
\end{align*}
\end{proof}



==> freq_unknown.tex <==
\subsection{Unknown Variance}
\label{sec:freq_unknown}

\red{Needs discussion!}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

%\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
%\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
%\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
%\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

%\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

%\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

